How does overparametrization affect performance on minority groups?

The benefits of overparameterization for the overall performance of modern machine learning (ML) models are well known. However, the effect of overparameterization at a more granular level of data subgroups is less understood. Recent empirical studies demonstrate encouraging results: (i) when groups are not known, overparameterized models trained with empirical risk minimization (ERM) perform better on minority groups; (ii) when groups are known, ERM on data subsampled to equalize group sizes yields state-of-the-art worst-group-accuracy in the overparameterized regime. In this paper, we complement these empirical studies with a theoretical investigation of the risk of overparameterized random feature models on minority groups. In a setting in which the regression functions for the majority and minority groups are different, we show that overparameterization always improves minority group performance.

==> YK-macros.tex <==

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\innerprod#1{\left\langle#1\right\rangle}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\st{\textrm{subject to}}
%\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> exps.tex <==
\section{Computational experiments}

\subsection{Synthetic experiment setup}
\paragraph{Data distribution}
We generate the data from two group model \eqref{eq:two-groups}. Among the total $n$ number of training points $\pi$ proportion of them belongs to the majority group $g = 1$ (\ie, \ $n_1 = \lfloor n\pi\rfloor$) and the rest are from the minority group $g = 0$ ($n_0 = n - \lfloor n\pi\rfloor$).

The features $x$ in each groups are $10$ dimensional vectors generated from multivariate standard normal distribution. The response are generated from \eqref{eq:two-groups} where $\beta_0$ and $\delta$ are specified as \[ \beta_0 = \frac{r_\beta}{\sqrt 5} (\mathbf{1}_5^T, \mathbf{0}_5^T)^T, \quad \delta = \frac{r_\delta}{\sqrt 5} (\mathbf{0}_5^T, \mathbf{1}_5^T)^T \]
In all our experiments we fix total number of training points $n$ to $900$ and the majority group proportion $\pi$ to $0.9.$ In the study of \emph{sub-population shift ratio} (SSR) (defined as $ r_{\beta:\delta} = r_\beta/r_\delta$) we fix $r_\beta = 5$ and $\sigma = 0.1.$ In the study of \emph{noise} ($\sigma$)  we fix $r_\beta = 5$ and $r_\delta = 1.$ 
\paragraph{Model}
In each of the setups we fit a neural net with single hidden layer $\text{ReLU}(Wx)\in \reals^p$, where $W\in\reals^{p \times 10}$ is a random matrix \cite{mei2019generalization}. Furthermore, the final layer doesn't have the bias variable (bias is set at zero). As one might see the only unknowns of this model are the weights of the final layer, which are obtained from ridgeless regression \cite{hastie2019Surprises} with $\text{ReLU}(Wx_i)$'s as features and $y_i$'s as responses. 

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{figs/ERM.pdf}
    \caption{\emph{Mean squared prediction error} (MSPE) of majority and minority groups are plotted against $\gamma = p/n$ (over 500 repetitions). The \emph{left} shows MSPE for several \emph{sub-population shift ratio} ($r_{\beta:\delta}$), whereas the same for different \emph{noise level} ($\sigma$) is shown \emph{right} panel.}
    \label{fig:mse-erm}
\end{figure}

% We generate data from the two groups model \eqref{eq:two-groups} wtih $\pi = 0.9$, $\Sigma = I_d$. In the first simulation, we set $\beta_0$ and $\beta_1 = \beta_0. \delta$ to be random unit vectors. We set $n = 200$ and vary $\gamma$ in $[1,10]$. Figure \ref{fig:bias} shows the (observed) bias and limiting bias \eqref{eq:limiting-bias} due to the difference between regression vectors. We see that the bias decreases as the aspect ratio $\gamma$ grows.

% \begin{figure}
%   \centering
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% %   \includegraphics[width=0.48\textwidth]{figs/bias-semilogy.png}
% %   ~
%   \includegraphics[width=0.48\textwidth]{figs/small-beta0-bias.png}
%   \caption{Bias and limiting bias \eqref{eq:limiting-bias} due to difference between regression vectors}
%   \label{fig:bias}
% \end{figure}

% In the second simulation, we generate set $\delta$ to be a random unit vector and study the prediction error with a small and a large values of $\beta_0$. The small $\beta_0$ setup is identical to the first simulation setup. In the large $\beta_0$ setup, we set $\beta_0$ to be a random norm 10 vector. The rest of the setup is identital to the first simulation setup. Figure \ref{fig:PE} shows the (observed) prediction error and limiting prediction error. We see that the prediction error decreases in the small $\beta_0$ setup, but it increases in the large $\beta_0$ setup.

% \begin{figure}
%   \centering
% %   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \includegraphics[width=0.48\textwidth]{figs/small-beta0-PE.png}
%   ~
%   \includegraphics[width=0.48\textwidth]{figs/big-beta0-PE.png}
%   \caption{Prediction error and limiting prediction error with a small (left) and large (right) value of $\beta_0$}
%   \label{fig:PE}
% \end{figure}


% \[
% \begin{aligned}
% \begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}^T(XX^T)^{-1}\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix} &= X_1^T(X_1(I - X_0^\dagger X_0)X_1^T)^{-1}X_1 \\
% &= X_1^T(X_1(I - \hSigma_0^\dagger\hSigma_0)X_1^T)^{-1}X_1 \\
% &= \lim\nolimits_{z\to 0_+}X_1^T(X_1(I - (\hSigma_0 + zI_d)^{-1}\hSigma_0)X_1^T)^{-1}X_1 \\
% &= \lim\nolimits_{z\to 0_+}X_1^T(zX_1(\hSigma_0 + zI_d)^{-1}X_1^T)^{-1}X_1 \\
% &= \lim\nolimits_{z\to 0_+}\frac1zX_1^T(X_1^\dagger)^T(\hSigma_0 + zI_d)X_1^\dagger X_1.
% \end{aligned}
% \]
% Thus the second term is
% \[
% \lim\nolimits_{z\to 0_+}\frac1z\tr(\tdelta_1\tdelta_1^T(\hSigma_0 + zI_d)),
% \]
% where $\tdelta_1 \triangleq X_1^\dagger X_1\delta$. 


% \subsection{Simulation2}
% We fit single hidden layer neural-net on data generated from linear regression setup. The two groups are indexed by $g\in \{1, -1\}$, $-1$ being the minority group. We fix $\beta = \text{SNR} \times  (1, 1, 1, 1, 1, 0, 0, 0, 0, 0)^T$ and $\delta = (0, 0, 0, 0, 0, 1, 1, 1, 1, 1)$. The pair $(x^{(g)}, y^{(g)})$ is generated from the following distribution. \begin{equation}
%     \left\{ \begin{aligned}
%     x^{(g)} & \sim N_{10}(0, I_{10})\\
%     y^{(g)} & \sim N\left(\left({x^{(g)}}\right)^T \beta_g, \sigma^2\right)
%     \end{aligned} \right.
% \end{equation} 
% The training data consists of 2000 independent pairs, where 90\% of them are from group 1 and 10\% are from group -1. We fit single hidden layer neural network with various number of nodes. NNs are trained with weighted sample points to account for class imbalance in training data. 
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\textwidth]{figs/plot.pdf}
%     \caption{Prediction error   }
%     \label{fig:mse-nn}
% \end{figure}


==> garbage.tex <==
\section{Extra}

\section{MSE for under-parameterizatized setting}
In the under-parameterized setting ($n>d$), we consider the least square estimator \[ \hat \beta = (X^TX)^{-1}X^Ty. \]
\begin{theorem}
Let $n, p \to \infty $ with $p/n\to \gamma \in (0, 1).$ Then \[
\text{MSPE} = \frac{\sigma^2 \gamma}{1-\gamma} + \frac{\pi\gamma\|\delta\|^2}{1-\gamma} + \frac{\pi^2 (1-2\gamma)\|\delta\|^2}{1-\gamma}. \]
\end{theorem}
\begin{proof}




The estimation error is \[
\begin{aligned}
\hat \beta - \beta_0 & =  (X^TX)^{-1}X^T(X\beta_0 + \begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + \eps) - \beta_0\\
& = (X^TX)^{-1}X^T\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + (X^TX)^{-1}X^T\eps
\end{aligned}
 \]
The MSPE is \[
\begin{aligned}
& \Ex\big[ (\hat \beta - \beta_0)^T(\hat \beta - \beta_0) \big]\\
& \quad = \Ex \left[ \delta^T \begin{bmatrix} 0_{n_0\times d} , X_1^T\end{bmatrix} X (X^TX)^{-2}X^T \begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta \right] + 2\Ex \big[ \delta^T \begin{bmatrix} 0_{n_0\times d}  X_1\end{bmatrix} X (X^TX)^{-2}X^T \eps \big]\\
& \quad \quad + \Ex \big[ \eps^T X(X^TX)^{-2}X^T\eps \big]
\end{aligned}
\]



To calculate the variance term we see that \[
\begin{aligned}
& \Ex \big[ \eps^T X(X^TX)^{-2}X^T\eps \big]\\
& \quad = \Ex \text{Tr}\big[ X(X^TX)^{-2}X^T\Ex_\eps(\eps \eps^T) \big]\\
& \quad = \sigma^2\Ex \text{Tr}\big[ (X^TX)^{-2}X^TX \big] \\
& \quad = \sigma^2\Ex \text{Tr}\big[ (X^TX)^{-1} \big] \\
& \quad = \sigma^2\frac{p}{n}\frac{1}{p}\Ex \text{Tr}\big[ (X^TX/n)^{-1} \big] \\
& \quad \to \sigma^2 \gamma \int \frac{1}{s}d\mu_\gamma(s)\\
&\quad = \frac{\sigma^2 \gamma}{1-\gamma}
\end{aligned}
\]
The covariance term $\Ex \big[ \delta^T \begin{bmatrix} 0_{n_0\times d}  X_1\end{bmatrix} X (X^TX)^{-2}X^T \eps \big]$ is zero. 

We now focus on the bias term. Note that, 
\[ \Ex \left[ \delta^T \begin{bmatrix} 0_{n_0\times d}  X_1^T\end{bmatrix} X (X^TX)^{-2}X^T \begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta \right] = \Ex \left[ \delta^T X_1^TX_1 (X^TX)^{-2}X_1^TX_1 \delta \right] \]
and for any $p \times p  $ orthogonal matrix $U$ \[ \Ex \left[ \delta^T X_1^TX_1 (X^TX)^{-2}X_1^TX_1 \delta \right] = \Ex \left[ \delta^TU^T X_1^TX_1 (X^TX)^{-2}X_1^TX_1 U\delta \right] \]
Letting $U$ be such an orthogonal matrix that $U\delta = \|\delta \|_2^2 e_i$ and averaging over $i = 1, 2, \dots, p$ we get \[
\begin{aligned}
\text{BIAS} &= \frac{\|\delta \|_2^2}{p}\Ex\left[ \text{Tr}\left\{ (X_1^TX_1)(X^TX)^{-2}(X_1^TX_1) \right\}\right]\\
&= \frac{\|\delta \|_2^2}{p}\Ex\left[ \text{Tr}\left\{ \left(\sum_{i=1}^{n_1}x_ix_i^T\right)^2(X^TX)^{-2} \right\}\right]\\
&= \frac{\|\delta \|_2^2}{p}\Ex\left[ \text{Tr}\left\{ \left(\sum_{i=1}^{n_1}\sum_{j=1}^{n_1}x_ix_i^Tx_jx_j^T\right)(X^TX)^{-2} \right\}\right]\\
&= \frac{\|\delta \|_2^2}{p} \Big[ n_1 \Ex \big[x_1^Tx_1 x_1^T(X^TX)^{-2}x_1\big] + n_1(n_1-1) \Ex \big[x_1^Tx_2 x_1^T(X^TX)^{-2}x_2\big] \Big]\\
&= \frac{\|\delta \|_2^2}{p} \big[ n_1 D_1 + n_1(n_1-1) D_2 \big]
\end{aligned}
\]

where the second last equality is obtained using exchangeability of $x_i$'s.

Using the above logic we get 
\begin{equation}
\label{eq:equality-D_1-D_2}
    n D_1 + n(n-1) D_2 = \Ex\Big[ \text{Tr}\big\{ (X^TX)(X^TX)^{-2}(X^TX) \big\}\Big] = p
\end{equation}

Let $A = X^T - x_1x_1^T.$ Hence \[
\begin{aligned}
x_1^T (A+x_1x_1^T)^{-2} x_1 &= x_1 ^T \left( A^{-1} - \frac{A^{-1}x_1x_1^T A^{-1}}{1+ x_1^TA^{-1}x_1}  \right) \left( A^{-1} - \frac{A^{-1}x_1x_1^T A^{-1}}{1+ x_1^TA^{-1}x_1}  \right) x_1\\
& = x_1^T A^{-1} \left( 1- \frac{x_1^T A^{-1}x_1}{1+x_1^2 A^{-1}x_1} \right)^2 A^{-1}x_1\\
& = \frac{x_1^TA^{-2}x_1}{(1+x_1^TA^{-1}x_1)^2}
\end{aligned}
\]

and \[ 
\begin{aligned}
D_1 & = \Ex \left[\frac{x_1^TA^{-2}x_1 x_1^T x_1}{(1+x_1^TA^{-1}x_1)^2}\right] \\
& = \Ex\left[ \frac{\frac{p^2}{(n-1)^2}\Big( x_1^T (A/(n-1))^{-2}x_1/p \Big) \Big( x_1^Tx_1/p \Big) }{\Big(1+\frac{p}{n-1}\big(x_1^T (A/(n-1))^{-1}x_1/p\big)\Big)^2}\right]\\
& \to \frac{\gamma^2 /(1-\gamma)^3}{\left(1+\gamma/(1-\gamma)\right)^2} = \frac{\gamma^2}{1-\gamma}
\end{aligned}
\] where the limit is obtained using lemmas \ref{lemma:p-conv} and \ref{lemma:moments-mp}. 

Using the equality \eqref{eq:equality-D_1-D_2} we get \[
D_2 = \frac{p - nD_1}{n(n-1)} \asymp \frac{\gamma - \frac{\gamma^2}{1-\gamma}}{n}  = \frac{\gamma(1-2\gamma)}{n(1-\gamma)}.
\]
Finally, we get \[
\begin{aligned}
\text{BIAS} &= \frac{\|\delta \|_2^2}{p} \big[ n_1 D_1 + n_1(n_1-1) D_2 \big]\\
& = \|\delta \|_2^2 \left[ \frac{\pi}{\gamma} \frac{\gamma^2}{1-\gamma} + \frac{\pi^2 }{\gamma}\frac{\gamma(1-2\gamma)}{1-\gamma}  \right]\\
& = \|\delta \|_2^2  \frac{\pi}{1-\gamma} (\gamma + \pi(1-2\gamma))
\end{aligned}
\]




\end{proof}

\begin{lemma}
\label{lemma:p-conv}
As $n, p\to \infty $ with $p/n \to \gamma\in (0, 1)$
\[
x_1^T (A/(n-1))^{-j}x_1/p \stackrel{p}{\to}\int \frac 1{s^{j}} d\mu_\gamma (s).  \]
\end{lemma}
\begin{proof}
We have \[
\begin{aligned}
\Ex \Big( x_1^T (A/(n-1))^{-j}x_1/p \Big) & = \frac{1}{p} \text{Tr} \Big((A/(n-1))^{-j}\Big)\\
\to \int \frac 1{s^{j}} d\mu_\gamma (s)
\end{aligned}
\] and \[
\begin{aligned}
\textbf{Var} \Big( x_1^T (A/(n-1))^{-j}x_1/p \Big) & = \frac{2}{p^2} \text{Tr} \Big((A/(n-1))^{-2j}\Big)\\
& \asymp\frac1p \int \frac 1{s^{2j}} d\mu_\gamma (s) \to 0
\end{aligned}
\]
\end{proof}

\begin{lemma}
\label{lemma:moments-mp}
For $0\le \gamma\le 1$ let $X\sim \mu_\gamma$ be a  Marchenko-Pastur random variable. Then \[ \Ex [1/X] = \frac{1}{1-\gamma}, \quad \Ex [1/X^2 ] = \frac{1}{(1-\gamma)^3}. \]
\end{lemma}

\begin{proof}
The Stieltjes transformation of $\mu_\gamma$ is \[
\begin{aligned}
s_\gamma(z) =&  \int \frac{1}{x - z}d\mu_\gamma(x)\\
=& \frac{1-\gamma - z - \sqrt{(1-\gamma- z)^2 - 4\gamma z}}{2\gamma z}, \quad z \in \bbC\backslash [1-\sqrt{\gamma}, 1+\sqrt{\gamma}].
\end{aligned}
 \]
 
 For $|z|< 1- \sqrt{\gamma}$
 \[
 \begin{aligned}
 s_\gamma(z) =&  \int \frac{1}{x - z}d\mu_\gamma(x)\\
=& \int \frac{1}{x}\frac{1}{1 - z/x}d\mu_\gamma(x)\\
=& \int \frac{1}{x}\sum_{k=0}^\infty (z/x)^k  d\mu_\gamma(x)
 \end{aligned}
 \]
 
 Hence, we have \[ \lim_{z\to 0+} s_\gamma (z) = \Ex[1/X], \quad \lim_{z\to 0+} \frac{d}{dz}\big(s_\gamma (z)\big) = \Ex[1/X^2]. \]
 
 Now, \[
 \begin{aligned}
 &1-\gamma -  z-\sqrt{(1-\gamma- z)^2 - 4\gamma z}\\ &\quad= 1-\gamma -  z-\big( 1+\gamma^2 + z^2 - 2\gamma - 2z + 2\gamma z - 4\gamma z \big)^{1/2} \\
 &\quad= 1-\gamma -  z-\big( (1-\gamma)^2 + z^2  - 2z - 2\gamma z  \big)^{1/2}\\
 &\quad \asymp 1-\gamma -  z-(1-\gamma) \Big[1+ \frac{z^2 -2z-2\gamma z}{2(1-\gamma)^2} - \frac{(z^2 -2z-2\gamma z)^2}{8(1-\gamma)^4}\Big],\quad \text{for }z \to 0+ \\
 &\quad \asymp 1-\gamma -  z-(1-\gamma) \Big[1+ \frac{z^2 -2z-2\gamma z}{2(1-\gamma)^2} - \frac{z^2(1+\gamma)^2}{2(1-\gamma)^4}\Big],\quad \text{for }z \to 0+ \\
 & \quad= \frac{z^2(1+\gamma)^2}{2(1-\gamma)^3}  - \frac{z^2-4\gamma z}{2(1-\gamma)} \\
 & \quad = \frac{2z^2 \gamma}{(1-\gamma)^3} + \frac{2\gamma z}{1-\gamma}
 \end{aligned}
 \]
 
which implies \[
\begin{aligned}
s_\gamma(z) \asymp \frac{z}{(1-\gamma)^3} + \frac{1}{1-\gamma}
\end{aligned}
\]
 This proves the lemma. 
\end{proof}


\section{Theory for general covariance matrix}

Let $ p/n \to \gamma \in (0,\infty). $ For a positive definite matrix $\Sigma_p \equiv \Sigma$ let $x  = \Sigma^{1/2}z$ where $z = (z_1, \dots , z_p)$ is a generic random vector which has \iid \  entries with \[
Ez_1 = 0, \quad Ez_1^2 = 1, \quad Ez_1^{12} \le B
\] for some positive number $B.$  We let $H_p$ to be the distribution of eigen-values   \ie\ $
H_p(s) = \frac1 p \sum_{i = 1}^p \delta_{s_i}(s),$  where  $s_1 \ge s_2 \ge \dots \ge s_p$ are eigen-values of $\Sigma.$ We assume $H_p$ converges weakly to $ H. $ For a measure $G$  we define the Stieltzes transform $ m_G(z) = \int \frac{1}{s-z}dG(s) $ and  the companion Stieltzes transform \[
\nu(z) + \frac1z = \gamma \left( m(z) + \frac1z \right).
\]
The Stieltzes transform can also be calculated from the following equation (\cite{ledoit2011eigenvectors}, Theorem 1) \[ m(z) = \int \frac{1}{s\big[1 - \gamma (1+zm(z))\big] - z}dH(s). \]
Define \[ \Theta_j (z) = \textbf{p-lim}_{n\to \infty} \frac1p \text{Tr}\big((\hat\Sigma - zI)^{-1} \Sigma^j\big). \]
It's obvious that $ m(z) = \Theta_0(z). $ From lemma 2 in \cite{ledoit2011eigenvectors} we get \[ \begin{aligned}
\Theta_1(z) &= \frac{1/\gamma^2}{1/\gamma - 1 - zm(z)} - \frac1\gamma \\
& = \frac1 \gamma \left(\frac{1}{1 - \gamma(1+zm(z)) } - 1\right)\\
& = \frac1\gamma \left( -\frac{1}{z\nu(z)} - 1 \right).
\end{aligned} \]


Also, from lemma 3 in \cite{ledoit2011eigenvectors} we have \[ \Theta_{k+1}(z) = \left[z\Theta_k(z) + \int s^kdH \right]\times \left[1+\gamma \Theta_1(z)\right]. \] These are the preliminary definitions and results required to prove the following theorem.

\begin{theorem}
Assume the prior $P_{\beta, \delta}$ for $\beta$ and $\delta$ with the following moments: \[E(\beta) = E(\delta) = 0, \quad E(\beta\beta^T) = \frac{r_\beta^2}p I, \quad E(\delta\delta^T) = \frac{r_\delta^2}p I, \quad E(\beta\delta^T) = \frac{r_{\beta, \delta}}p I \] 
\[  
R(\hat \beta)  \to \begin{cases} \frac{r_\beta^2}{\gamma \nu(0)} + \frac{r_\delta^2\pi}{\gamma\nu(0)}\left(\gamma \nu(0)\int s dH - 1\right)  \left[   (1-\pi)\gamma \nu(0)\int s dH   +   \pi   \right]
 & \text{for } \gamma > 1\\
 \quad  + \sigma^2 \left(\frac{\nu'(0)}{\nu^2(0)}-1\right)\\
 \frac{r_\delta^2\pi}{\gamma(1-\gamma)} \int sdH \big[ \gamma^2 + \pi\gamma (1-2\gamma) \big] + \sigma^2 \frac\gamma{1-\gamma}
  & \text{for } \gamma < 1
 \end{cases} 
\] 

\end{theorem}


\begin{proof}
	The estimation error 
	\[
	\begin{aligned}
	\hat \beta - \beta_0 & =  (X^TX)^{+}X^T(X\beta_0 + \begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + \eps) - \beta_0\\
	& = \big((X^TX)^{+}X^TX - I\big)\beta_0   + (X^TX)^{+}X^T\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + (X^TX)^{+}X^T\eps\\
	& = \big(X^T(XX^T)^{-1}X - I\big)\beta_0   + X^T(XX^T)^{-1}\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + (X^TX)^{+}X^T\eps
	\end{aligned}
	\]
Let us define $ \Pi = (X^TX)^+ X^TX .$	The MSPE is 
	\[
	\begin{aligned}
	R(\hat\beta) & = E\big[  (\hat \beta - \beta_0)^T \Sigma (\hat \beta - \beta_0) \big] \\
	& = E \big[  \beta_0^T (I - \Pi ) \Sigma (I-\Pi)\beta_0  \big] + E\big[ \eps^T X (X^TX)^{+} \Sigma (X^TX)^{+} X^T \eps  \big] \\
	& \quad + E\big[  \delta^T X_1^TX_1 (X^TX)^{+} \Sigma (X^TX)^{+} X_1^T X_1 \delta  \big]\\
	& \quad - 2 E \Big[ \beta_0^T (I - \Pi ) \Sigma (X^TX)^{+}X^T\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta  \Big]\\
	& \quad = B(\hat \beta) + V(\hat\beta) + B_2(\hat \beta) - 2C(\hat \beta)
	\end{aligned}
	\]
	\paragraph{Calculation of $B(\hat \beta)$}
	
	If $\gamma >1$
	\[
	\begin{aligned}
	(I - \Pi ) \Sigma (X^TX)^{+}X^T & = (I - X^T (XX^T)^{-1}X ) \Sigma X^T(XX^T)^{-1}
	\end{aligned}
	\]
	
	
	\[
	\begin{aligned}
	B(\hat \beta ) & = E\big[ \beta_0 ^T (I - \Pi) \Sigma (I - \Pi) \beta_0 \big]\\
	& = \frac{\|\beta_0 \|_2^2}{p} E\big[\text{Tr} \big((I-\Pi)\Sigma (I-\Pi)\big) \Big] \\
	& = r_\beta^2 E\Big[\frac1p\text{Tr} \big((I - \Pi)\Sigma\big)  \Big]\\
	& = \frac{r_\beta^2}{\gamma \nu(0-)}
	\end{aligned}
	\]
	since
	\[
	\begin{aligned}
	\frac1p\text{Tr} \big((I - \Pi)\Sigma\big) & = \lim_{z\to 0+} \frac1p\text{Tr} \big[(I - (X^TX+nzI)^{-1}(X^TX))\Sigma\big]\\
	& = \lim_{z\to 0+}  \frac{nz}{p} \text{Tr} \big[ (X^TX+nzI)^{-1}\Sigma\big]\\
	& = \lim_{z\to 0+}  \frac{z}{p} \text{Tr} \big[ (X^TX/n+zI)^{-1}\Sigma\big]\\
	& = \lim_{z\to 0+}  \frac{z}{p} \text{Tr} \big[ (\hat \Sigma+zI)^{-1}\Sigma\big]\\
	& \to \lim_{z\to 0+} z \Theta_1(-z)\\
	& = \lim_{z\to 0+} z \frac1 \gamma \left(-1 + \frac{1}{z\nu(-z)}\right)\\
	& = \frac{1}{\gamma \nu(0-)}
	\end{aligned}
	\]
	If $\gamma < 1$ we have $B(\hat \beta )  = 0.$
	
	
	\paragraph{Calculation of $V(\hat \beta)$}
	If $\gamma >1$ then 
	\[
	\begin{aligned}
	 V(\hat \beta)& = E\big[ \eps^T X (X^TX)^{+} \Sigma (X^TX)^{+} X^T \eps  \big] \\
	 & = \sigma^2 E\Big[\text{Tr}\big\{  (X^TX)^{+} \Sigma (X^TX)^{+} X^T X  \big\}\Big]\\
	&  = \sigma^2 \lim_{z\to 0+} E\Big[\text{Tr}\big\{  (X^TX+nzI)^{-1} \Sigma (X^TX+nzI)^{-1} X^T X  \big\}\Big]\\
	&  = \sigma^2\frac1 n \lim_{z\to 0+} E\Big[\text{Tr}\big\{  (X^TX/n+zI)^{-1} \Sigma (X^TX/n+zI)^{-1} (X^T X/n)  \big\}\Big]\\
	&  = \sigma^2\gamma \lim_{z\to 0+}\frac1 p E\Big[\text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma (\hat \Sigma+zI)^{-1} \hat \Sigma  \big\}\Big]\\
	& = \sigma^2 \left( \frac{\nu'(0)}{\nu^2(0)} -1 \right)
	\end{aligned}
	\]
	since, 
	\[
	\begin{aligned}
	& \lim_{z\to 0+}\frac1 p \text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma (\hat \Sigma+zI)^{-1} \Sigma  \big\}\\
	& \quad = \lim_{z\to 0+}\left[\frac1 p \text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma  \big\} - z \frac 1p\text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma (\hat \Sigma+zI)^{-1}   \big\}\right]\\
	& \quad = \lim_{z\to 0+}\left[\frac1 p \text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma  \big\} - z \frac 1p\text{Tr}\big\{  (\hat \Sigma+zI)^{-2} \Sigma    \big\}\right]\\
	& \quad = \lim_{z\to 0+}\left[\frac1 p \text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma  \big\} + z \frac{d}{dz}\left(\frac 1p\text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma    \big\}\right)\right]\\
	& \quad \to \lim_{z\to 0+} \big( \Theta_1(-z) + z \Theta_1'(-z) \big)\\
	& \quad = \lim_{z\to 0+} \big( z\Theta_1(-z)  \big)'\\
	& \quad = \lim_{z\to 0+}\frac 1 \gamma \big( -z + \frac 1{\nu(-z)}  \big)'\\
	& \quad = \lim_{z\to 0+} \frac{1}{\gamma} \left(-1 + \frac{\nu'(-z)}{\nu^2(-z)} \right)\\
	& \quad = \frac{1}{\gamma} \left(-1 + \frac{\nu'(0)}{\nu^2(0)} \right)
	\end{aligned}
	\]
	
	If $\gamma < 1$ then \[
	\begin{aligned}
	V(\hat \beta)
	 & = \sigma^2 E\Big[\text{Tr}\big\{  (X^TX)^{+} \Sigma (X^TX)^{+} X^T X  \big\}\Big]\\
	 & = \sigma^2 E\Big[\text{Tr}\big\{  (X^TX)^{-1} \Sigma   \big\}\Big]\\
	 & = \sigma^2 E\Big[\text{Tr}\big\{  \big(\Sigma^{-1/2}X^TX\Sigma^{-1/2}\big)^{-1}   \big\}\Big]\\
	 & = \sigma^2 \frac1n E\Big[\text{Tr}\big\{  \big(Z^TZ/n\big)^{-1}   \big\}\Big]\\
	 & = \sigma^2 \gamma \frac1p  E\Big[\text{Tr}\big\{  \big(Z^TZ/n\big)^{-1}   \big\}\Big]\\
	 & = \sigma^2 \frac\gamma{1-\gamma}
	\end{aligned}
	\]
	\paragraph{\underline{Calculation of $B_2(\hat \beta)$}}
	For $\gamma>1$
	\[
	\begin{aligned}
	B_2(\hat \beta) & = E\big[  \delta^T X_1^TX_1 (X^TX)^{+} \Sigma (X^TX)^{+} X_1^T X_1 \delta  \big]\\
	& = \frac{r_\delta^2}{p} E\big[ \text{Tr} \big\{  X_1^TX_1 (X^TX)^{+} \Sigma (X^TX)^{+} X_1^T X_1 \big\}  \big]\\
	& = \frac{r_\delta^2}{p} E\left[ \sum_{i,j = 1}^{n_1} \text{Tr} \big\{  x_ix_i^T  (X^TX)^{+} \Sigma (X^TX)^{+} x_j x_j^T \big\}  \right]\\
	& = n_1\frac{r_\delta^2}{p} E\left[ x_1^T  x_1x_1^T  (X^TX)^{+} \Sigma (X^TX)^{+} x_1  \right]\\
	& \quad  + n_1(n_1 - 1)\frac{r_\delta^2}{p} E\left[ x_1^T  x_2x_1^T  (X^TX)^{+} \Sigma (X^TX)^{+} x_2  \right]\\
	& = \frac{r_\delta^2}{p} \big[n_1 D_1 + n_1(n_1-1)D_2 \big]
	\end{aligned}
	\]
	
	
	\[
	\begin{aligned}
	D_1 & =  (x_1^T x_1)  x_1^T  (X^TX)^{+} \Sigma (X^TX)^{+} x_1\\
	&  = \lim_{z\to 0+} x_1^T x_1  x_1^T  (X^TX + (n-1)zI)^{-1} \Sigma (X^TX + (n-1)zI)^{-1} x_1 \\
	&  = \lim_{z\to 0+} (x_1^T x_1)  x_1^T  ( x_1x_1^T +  X_{-1}^TX_{-1} + (n-1)zI)^{-1} \Sigma (x_1x_1^T + X_{-1}^TX_{-1} + (n-1)zI)^{-1} x_1\\
	&  = \lim_{z\to 0+}(x_1^T x_1)   x_1^T  \left(A^{-1} - \frac{A^{-1} x_1 x_1 ^T A^{-1}}{1 + x_1^TA^{-1}x_1}\right)  \Sigma \left(A^{-1} - \frac{A^{-1} x_1 x_1 ^T A^{-1}}{1 + x_1^TA^{-1}x_1}\right) x_1,\quad \text{where } A = X_{-1}^T X_{-1} + (n-1)zI, \\
	&  = \lim_{z\to 0+} \frac{(x_1^T x_1) x_1^T A^{-1}\Sigma A^{-1}x_1}{(1+x_1^TA^{-1}x_1)^2}\\
	&  = \lim_{z\to 0+} \frac{(x_1^T x_1) \frac 1 {(n-1)^2} x_1^T (\hat \Sigma' + zI )^{-1}\Sigma (\hat \Sigma' + zI)^{-1}x_1}{\left(1+\frac1 {n-1}x_1^T(\hat \Sigma' + zI )^{-1}x_1\right)^2}\\
	&  = \lim_{z\to 0+} \frac{\gamma^2(\frac1p x_1^T x_1) \frac 1 {p} x_1^T z^2 (\hat \Sigma' + zI )^{-1}\Sigma (\hat \Sigma' + zI)^{-1}x_1}{\left(z+\gamma\frac1 {p}x_1^Tz(\hat \Sigma' + zI )^{-1}x_1\right)^2}
	\end{aligned}
	\] where $ \hat \Sigma' = X_{-1}^TX_{-1}/(n-1). $
	Using lemma \ref{lemma:conv-parts} we get \[ 
	\begin{aligned}
	D_1 & = \lim_{z\to 0+} \frac{\gamma^2(\frac1p x_1^T x_1) \frac 1 {p} x_1^T z^2 (\hat \Sigma' + zI )^{-1}\Sigma (\hat \Sigma' + zI)^{-1}x_1}{\left(z+\gamma\frac1 {p}x_1^Tz(\hat \Sigma' + zI )^{-1}x_1\right)^2} \\
	& \to \lim_{z\to 0+} \frac{\left(\int s dH\right)z^2\gamma^2 \big(- \Theta_2(-z)\big)'}{\big(z+\gamma z\Theta_1(-z)\big)^2}\\
	& = \lim_{z\to 0+} \frac{\left(\int s dH\right)z^2\gamma^2 \frac{d}{dz}\left[\left( z\Theta_1(-z) - \int s dH\right)\left(1 + \gamma\Theta_1(-z)\right)\right]}{\big(z+\gamma z\Theta_1(-z)\big)^2}\\
	& = \lim_{z\to 0+} \frac{\gamma\left(\int s dH\right)z^2 \frac{d}{dz}\left[\left( \gamma z\Theta_1(-z) - \gamma \int s dH\right)\left(1  + \gamma\Theta_1(-z)\right)\right]}{\gamma\big(z+\gamma z\Theta_1(-z)\big)^2}\\
	& = \lim_{z\to 0+} \frac{\gamma\left(\int s dH\right)z^2 \frac{d}{dz}\left[\left( -z + \frac 1{\nu(-z)} - \gamma \int s dH\right)\left( \frac{1}{ z \nu(-z)} \right)\right]}{\big(\frac1{\nu(-z)}\big)^2}\\
	& = \lim_{z\to 0+} \gamma \left(\int s dH\right)z^2 \nu^2 (-z) \left[\left( -1 + \frac {\nu'(-z)}{\nu^2(-z)} \right)\left( \frac{1}{ z \nu(-z)}  \right)\right.\\
	& \quad\quad\quad   + \left. \left( -z + \frac 1{\nu(-z)} - \gamma \int s dH\right)\left(- \frac{1}{ z^2 \nu(-z)} +\frac {\nu'(-z)}{ z\nu^2(-z)} \right) \right]\\
	& = \gamma\left(\int s dH\right) \nu^2(0) \left(\gamma \int s dH  - \frac1 {\nu(0)}\right)\frac1{ \nu(0)}\\
	& = \gamma \left(\int s dH\right)  \left(\gamma \nu(0)\int s dH - 1\right)
	\end{aligned} \]


	We also notice
	\[ \text{Tr} \big\{  x_1x_1^T (X^TX)^{+} \Sigma (X^TX)^{+} (X^T X) \big\} = D_1 + (n-1)D_2. \] We shall try to compute the in probability limit of the term $ \text{Tr} \big\{  x_1x_1^T (X^TX)^{+} \Sigma (X^TX)^{+} (X^T X) \big\} $ which shall provide the same for $ D_2. $
	
	Note that
	 \[ \begin{aligned}
	& \text{Tr} \big\{  x_1x_1^T (X^TX)^{+} \Sigma (X^TX)^{+} (X^T X) \big\}\\
	& \quad = \lim_{z\to 0+} \text{Tr} \big\{  x_1x_1^T (X^TX + (n-1)zI)^{-1} \Sigma (X^TX + (n-1)zI)^{-1} (X^T X) \big\}\\
	& \quad = \lim_{z\to 0+}x_1^T (X^TX + (n-1)zI)^{-1} \Sigma (X^TX + (n-1)zI)^{-1} (X^T X) x_1\\
	& \quad = \lim_{z\to 0+}\left[x_1^T (X^TX + (n-1)zI)^{-1} \Sigma  x_1\right.\\
	& \quad \quad \quad\left. - (n-1)zx_1^T (X^TX + (n-1)zI)^{-1} \Sigma (X^TX + (n-1)zI)^{-1}  x_1 \right]
	\end{aligned}\]
	Now, \[ \begin{aligned}
	& \lim_{z\to 0+} x_1^T (X^TX + (n-1)zI)^{-1} \Sigma  x_1\\
	& \quad = \lim_{z\to 0+} x_1^T \big(x_1 x_1^T + X_{-1}^TX_{-1} + (n-1)zI\big)^{-1} \Sigma  x_1\\
	& \quad = \lim_{z\to 0+} x_1^T \left(\big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1}\right.\\
	&\quad \quad \quad\left. -\frac{ \big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1}x_1x_1^T\big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1}}{1 + x_1^T\big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1}x_1}\right) \Sigma  x_1\\
	& \quad = \lim_{z\to 0+}\frac{x_1^T\big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1}\Sigma x_1}{1+ x_1^T\big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1} \Sigma  x_1}\\
	& \quad = \lim_{z\to 0+}\frac{\frac1{n-1}x_1^T\big( \hat \Sigma' + zI\big)^{-1}\Sigma x_1}{1+ \frac1{n-1}x_1^T\big( \hat \Sigma' + zI\big)^{-1} \Sigma  x_1}\\
	& \quad = \lim_{z\to 0+}\frac{\gamma z\frac1{p}x_1^T\big( \hat \Sigma' + zI\big)^{-1}\Sigma x_1}{z+ \gamma z\frac1{p}x_1^T\big( \hat \Sigma' + zI\big)^{-1} \Sigma  x_1}\\
	& \quad \to \lim_{z\to 0+}\frac{\gamma z\Theta_2(-z)}{z+ \gamma z\Theta_1(-z)}\\
	& \quad = \lim_{z\to 0+}\frac{\gamma z\left(\int s dH - z\Theta_1(-z)\right)\left(1+\gamma \Theta_1(z)\right)}{\frac1{\nu(-z)}}\\
	& \quad = \lim_{z\to 0+}\nu(-z) \left(\gamma \int s dH - \gamma z\Theta_1(-z)\right)\left(z+z\gamma \Theta_1(z)\right)\\
	& \quad = \lim_{z\to 0+}\nu(-z) \left(\gamma \int s dH - \frac1 {\nu(-z)} + z\right)\left( \frac{1}{ \nu(-z)} \right)\\
	& \quad \to \nu(0) \left(\gamma \int s dH - \frac1 {\nu(0)} \right)\frac{1}{ \nu(0)}\\
	& \quad = \frac{1}{ \nu(0)} \left(\gamma \int s dH \nu(0)-1 \right)
	\end{aligned} \]
	
	and \[ \begin{aligned}
	& \lim_{z\to 0+} (n-1)zx_1^T (X^TX + (n-1)zI)^{-1} \Sigma (X^TX + (n-1)zI)^{-1}  x_1\\
	& \quad = \lim_{z\to 0+} \frac1{n-1}zx_1^T (\hat\Sigma + zI)^{-1} \Sigma (\hat\Sigma + zI)^{-1}  x_1\\
	& \quad = 0
	\end{aligned} \]
	where the limit is zero because $  \frac1{n-1}x_1^T (\hat\Sigma + zI)^{-1} \Sigma (\hat\Sigma + zI)^{-1}  x_1 $ converges to a finite limit. 
	
	Hence, we get \[ 
	\begin{aligned}
	(n-1)D_2 &= \frac{1}{ \nu(0)} \left(\gamma \int s dH \nu(0)-1 \right) - \gamma \left(\int s dH\right)  \left(\gamma \nu(0)\int s dH - 1\right)\\
	& = -\frac{1}{ \nu(0)} \left(\gamma \nu(0)\int s dH - 1\right)^2
	\end{aligned} \]
	Finally, we get \[ \begin{aligned}
	B_2(\hat \beta) 
	& = \frac{r_\delta^2}{p} \big[n_1 D_1 + n_1(n_1-1)D_2 \big]\\
	& \asymp r_\delta^2 \left[\frac\pi\gamma  D_1 + \frac{\pi^2}\gamma (n-1) D_2 \right]\\
	& \asymp r_\delta^2 \left[  \frac\pi\gamma \gamma \left(\int s dH\right)  \left(\gamma \nu(0)\int s dH - 1\right) - \frac{\pi^2} \gamma \frac{1}{ \nu(0)} \left(\gamma \nu(0)\int s dH - 1\right)^2  \right]\\
	& = \frac{r_\delta^2\pi}{\gamma\nu(0)}\left(\gamma \nu(0)\int s dH - 1\right)  \left[   \left(\gamma \nu(0)\int s dH\right)   - \pi  \left( \gamma\nu(0)\int s dH - 1\right)  \right]\\
	& = \frac{r_\delta^2\pi}{\gamma\nu(0)}\left(\gamma \nu(0)\int s dH - 1\right)  \left[   (1-\pi)\gamma \nu(0)\int s dH   +   \pi   \right]
	\end{aligned} \]
\end{proof}


\begin{lemma}[\cite{ledoit2011eigenvectors}, lemma 1]
	\label{lemma:conv-quadratic-exp}
	Let $Y = (y_1, \dots, y_N)$ be a random vector with \iid\ entries satisfying:
	\[ E y_1 = 0, \quad E y_1^2 = 1, \quad Ey_1^{12} \le B  \] where the constant $ B $ doesn't depend on $ N .$ Let also $ A $ be a $ N \times N $ matrix. Then there exists a constant $ K>0 $ independent of $ Y, A, N $ such that: \[
	E\left|  Y^T AY - \text{Tr} (A) \right|^6 \le K\|A\|_{\text{op}} N^3.
	\] 
	Furthermore, if $ \|A\|_{\text{op}} N^3 \to 0  $ as $ N\to \infty $ then \[
	Y^T AY -  \text{Tr} (A)\to 0  \text{ in probability.}
	\] 
\end{lemma}


\begin{lemma}
	\label{lemma:conv-parts}
	The following in probability convergence holds: 
	\begin{enumerate}
		\item $ \frac1 p x_1^Tx_1 \to \int s dH, $
		\item $ \frac1 {p}x_1^Tz(\hat \Sigma + zI )^{-1}\Sigma^j x_1 \to z \Theta_{j+1}(-z),  $
		\item $ \frac 1 {p} x_1^T z^2 (\hat \Sigma + zI )^{-1}\Sigma (\hat \Sigma + zI)^{-1}x_1 \to z^2 (-\Theta_2(-z))' $
	\end{enumerate}
	
\end{lemma}


	We shall use \ref{lemma:conv-parts} repeatedly. 
	
	
	\textbf{(1)} Note that $ \frac1 p x_1^Tx_1 = z_1^T (\Sigma/p) z_1. $ Here $ \|\Sigma/p\|_{\text{op}} p^3 = \sigma_{\text{max}} \frac{\sigma_{\text{max}}^6}{p^3} \to 0. $ Hence, \[ 
	\frac1 p x_1^Tx_1  - \int s dH = \frac1 p x_1^Tx_1 -   \text{Tr} (\Sigma/p) + \frac1p  \text{Tr} (\Sigma) - \int s dH \to 0.
	\]
	
	\textbf{(2)} Here $  \frac1 {p}x_1^Tz(\hat \Sigma + zI )^{-1}\Sigma^j x_1 =  z_1^T\left(\frac{\Sigma ^{1/2}(z\hat \Sigma + I )^{-1}\Sigma ^{1/2+j}}{p}\right)z_1 $ and \[ 
	\begin{aligned}
	\left\|\frac{\Sigma ^{1/2}(\hat \Sigma/z + I )^{-1}\Sigma ^{1/2+j}}{p}\right\|_{\text{op}} & \le \frac1p \|\Sigma^{1/2}\|_{\text{op}}  \|(\hat \Sigma/z + I )^{-1}\|_{\text{op}} \|\Sigma^{1/2+j}\|_{\text{op}} \\
	&\le  \frac{\sigma_{\text{max}}}{p}^{j+1}
	\end{aligned} \] This implies \[	\left\|\frac{\Sigma ^{1/2}(\hat \Sigma/z + I )^{-1}\Sigma ^{1/2+j}}{p}\right\|_{\text{op}}^{6+6j} p^3 \to 0,   \] and we get \[ 
	\frac1 {p}x_1^Tz(\hat \Sigma + zI )^{-1}\Sigma^jx_1 - \text{Tr} \left(\frac{\Sigma ^{1/2}z(\hat \Sigma + zI )^{-1}\Sigma ^{1/2+j}}{p}\right) \to 0
	\]in probability. Since, \[ \text{Tr} \left(\frac{\Sigma ^{1/2}z(\hat \Sigma + zI )^{-1}\Sigma ^{1/2+j}}{p}\right) \to z \Theta_{j+1}(-z) \] in probability, we have the result. 
	
	\textbf{(3)} Note that \[ \begin{aligned}
	& \frac 1 {p} x_1^T z^2 (\hat \Sigma + zI )^{-1}\Sigma (\hat \Sigma + zI)^{-1}x_1\\
	&\quad  = \frac 1 {p} z_1^T \Sigma^{1/2} z^2 \Sigma^{-1/2} \big(\Sigma^{-1/2}\hat \Sigma \Sigma^{-1/2} + z\Sigma^{-1} \big)^{-1}\Sigma^{-1/2}\Sigma\Sigma^{-1/2} \big(\Sigma^{-1/2}\hat \Sigma\Sigma^{-1/2} + z\Sigma^{-1}\big)^{-1}\Sigma^{-1/2}\Sigma^{1/2}z_1\\
	& \quad = \frac 1 {p} z_1^T  z^2  \big(\Sigma^{-1/2}\hat \Sigma \Sigma^{-1/2} + z\Sigma^{-1} \big)^{-2} z_1\\
	& \quad =  z_1^T \left(\frac{   \Sigma\big(\hat \Sigma/z  + I \big)^{-2}\Sigma}{p}\right) z_1
	\end{aligned} \] and \[ \begin{aligned}
	\left\|\frac{   \Sigma\big(\hat \Sigma/z  + I \big)^{-2}\Sigma}{p} \right\|_{\text{op}} \le \frac1 p \sigma_{\text{max}}^2 .
	\end{aligned} \] This implies \[ \left\|\frac{   \Sigma\big(\hat \Sigma/z  + I \big)^{-2}\Sigma}{p} \right\|_{\text{op}}^6 p^3 \le \frac 1{p^3} \sigma_{\text{max}}^{12}\to 0 \] which gives us \[ \frac 1 {p} x_1^T z^2 (\hat \Sigma + zI )^{-1}\Sigma (\hat \Sigma + zI)^{-1}x_1 - \text{Tr}\left(\frac{   \Sigma\big(\hat \Sigma/z  + I \big)^{-2}\Sigma}{p}\right) \to 0 \] in probability. Since, \[ \begin{aligned}
	\text{Tr}\left(\frac{   \Sigma^{1/2}\big(\hat \Sigma/z  + I \big)^{-2}\Sigma^{1/2}}{p}\right) &= \frac{z^2}{p}\text{Tr}\left(   \big(\hat \Sigma/z  + I \big)^{-2}\Sigma^2\right)\\
	& = - z^2\frac{d}{dz}\left(\frac1p\text{Tr}\left(   \big(\hat \Sigma/z  + I \big)^{-1}\Sigma^2\right)  \right)\\
	& \to - z^2 \frac{d}{dz} \big(\Theta_2(-z)\big)
	\end{aligned} \] in probability, we have the result.
	
	
	For $\gamma<1$ we note that 
	
	\[m(0) = \int\frac1s dG_{X^TX/n} (s), \quad m'(0) =\int\frac1{s^2} dG_{X^TX/n} (s)  \] are finite quantities. Hence from  \[ \begin{aligned}
\Theta_1(z) &= \frac{1/\gamma^2}{1/\gamma - 1 - zm(z)} - \frac1\gamma \\
& = \frac1 \gamma \left(\frac{1}{1 - \gamma(1+zm(z)) } - 1\right)
\end{aligned} \] we get \[ \Theta_1(-z) = \frac1{1-\gamma} \] as $z \to 0+.$

\[
	\begin{aligned}
	D_1 & =  (x_1^T x_1)  x_1^T  (X^TX)^{-1} \Sigma (X^TX)^{-1} x_1\\
    &  = (x_1^T x_1)   x_1^T  \left(A^{-1} - \frac{A^{-1} x_1 x_1 ^T A^{-1}}{1 + x_1^TA^{-1}x_1}\right)  \Sigma \left(A^{-1} - \frac{A^{-1} x_1 x_1 ^T A^{-1}}{1 + x_1^TA^{-1}x_1}\right) x_1,\\
	&\quad\quad \text{where } A = X_{-1}^T X_{-1}, \\
	&  =  \frac{(x_1^T x_1) x_1^T A^{-1}\Sigma A^{-1}x_1}{(1+x_1^TA^{-1}x_1)^2}\\
	&  =  \frac{(x_1^T x_1) \frac 1 {(n-1)^2} x_1^T (\hat \Sigma'  )^{-1}\Sigma (\hat \Sigma' )^{-1}x_1}{\left(1+\frac1 {n-1}x_1^T(\hat \Sigma'  )^{-1}x_1\right)^2}\\
	&  =  \frac{\gamma^2(\frac1p x_1^T x_1) \frac 1 {p} x_1^T  (\hat \Sigma' )^{-1}\Sigma (\hat \Sigma' )^{-1}x_1}{\left(1+\gamma\frac1 {p}x_1^T(\hat \Sigma' )^{-1}x_1\right)^2}\\
	& \to \frac{\gamma^2\left(\frac1 p \text{Tr}(\Sigma)\right)\left( \frac 1 {p} \text{Tr}\big(\Sigma  (\hat \Sigma' )^{-1}\Sigma (\hat \Sigma' )^{-1}\big)\right)}{\left(1+\gamma\frac1 {p}\text{Tr}\big(\Sigma\hat (\Sigma')^{-1} \big)\right)^2}
	\end{aligned}
	\]

Here $\frac1p\text{Tr}(\Sigma) \to \int sdH $, \[
\begin{aligned}
\frac1 {p}\text{Tr}\big(\Sigma\hat (\Sigma')^{-1} \big) & = \frac1 {p}\text{Tr}\big(\hat (\Sigma^{-1/2}\Sigma'\Sigma^{-1/2})^{-1} \big)\\
& = m_{I}(0) = \frac1{1-\gamma}
\end{aligned}
\] and 
\[
\begin{aligned}
\frac 1 {p} \text{Tr}\big(\Sigma  (\hat \Sigma' )^{-1}\Sigma (\hat \Sigma' )^{-1}\big) & = \frac1 {p}\text{Tr}\big( (\Sigma^{-1/2}\Sigma'\Sigma^{-1/2})^{-2} \big)\\
& = m_{I}'(0) = \frac1{(1-\gamma)^3}
\end{aligned}
\] where $m_I$ is the Stieltzes transform with $\Sigma = I.$ 
Hence, \[
\begin{aligned}
D_1 & \to \frac{\gamma^2\int sdH\frac1{(1-\gamma)^3}}{\left(1+\frac\gamma{(1-\gamma)}\right)^2}\\
& = \frac{\gamma^2}{1-\gamma}\int sdH
\end{aligned}
\] Furthermore, 
\[
\begin{aligned}
& D_1 + (n-1)D_2 \\
& \quad = \gamma\frac1p \big(nD_1 + n(n-1)D_2\big) \\
&\quad = \gamma\frac1p \text{Tr} \big\{  X^TX (X^TX)^{-1} \Sigma (X^TX)^{-1} (X^T X) \big\}\\
& \quad =\gamma \frac{1}{p}\text{Tr}(\Sigma)\\
& \quad \to \gamma\int sdH
\end{aligned}
\]
Hence \[ (n-1)D_2 = \gamma\int sdH - \frac{\gamma^2}{1-\gamma}\int sdH = \gamma\left(\frac{1-2\gamma}{1-\gamma}\right)\int sdH.\]

Hence, \[
\begin{aligned}
B_2(\hat\beta) &  = \frac{r_\delta^2}{p} \big[n_1 D_1 + n_1(n_1-1)D_2 \big]\\
& \asymp r_\delta^2\frac\pi\gamma \left(\frac{\gamma^2}{1-\gamma}\int sdH + \pi (n-1)D_2 \right)\\
& \asymp r_\delta^2\frac\pi\gamma \left(\frac{\gamma^2}{1-\gamma}\int sdH + \pi \gamma\left(\frac{1-2\gamma}{1-\gamma}\right)\int sdH \right)\\
& = \frac{r_\delta^2\pi}{\gamma(1-\gamma)} \int sdH \big[ \gamma^2 + \pi\gamma (1-2\gamma) \big]
\end{aligned}
\]

\paragraph{Calculation of $C(\hat \beta)$}
If $\gamma>1$ then 
\[
\begin{aligned}
& E \Big[ \beta_0^T (I - \Pi ) \Sigma (X^TX)^{+}X^T\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta  \Big] \\
&\quad = \frac{n_1}n E \Big[ \beta_0^T (I - \Pi ) \Sigma (X^TX)^{+}X^TX\delta  \Big]\\
&\quad = \pi r_{\beta, \delta} E \left[\text{Tr}\Big[  (I - \Pi ) \Sigma \Pi  \Big]\right]\\
&\quad =0
\end{aligned}
\]
If $\gamma < 1$ then $\Pi = I$ and hence $C(\hat \beta) = 0.$


==> gen-theory.tex <==
\section{Theory for general covariance matrix}

Let $ p/n \to \gamma \in (0,\infty). $ For a positive definite matrix $\Sigma_p \equiv \Sigma$ let $x  = \Sigma^{1/2}z$ where $z = (z_1, \dots , z_p)$ is a generic random vector which has \iid \  entries with \[
Ez_1 = 0, \quad Ez_1^2 = 1, \quad Ez_1^{12} \le B
\] for some positive number $B.$  We let $H_p$ to be the distribution of eigen-values   \ie\ $
H_p(s) = \frac1 p \sum_{i = 1}^p \delta_{s_i}(s),$  where  $s_1 \ge s_2 \ge \dots \ge s_p$ are eigen-values of $\Sigma.$ We assume $H_p$ converges weakly to $ H. $ For a measure $G$  we define the Stieltzes transform $ m_G(z) = \int \frac{1}{s-z}dG(s) $ and  the companion Stieltzes transform \[
\nu(z) + \frac1z = \gamma \left( m(z) + \frac1z \right).
\]
The Stieltzes transform can also be calculated from the following equation (\cite{ledoit2011eigenvectors}, Theorem 1) \[ m(z) = \int \frac{1}{s\big[1 - \gamma (1+zm(z))\big] - z}dH(s). \]
Define \[ \Theta_j (z) = \textbf{p-lim}_{n\to \infty} \frac1p \text{Tr}\big((\hat\Sigma - zI)^{-1} \Sigma^j\big). \]
It's obvious that $ m(z) = \Theta_0(z). $ From lemma 2 in \cite{ledoit2011eigenvectors} we get \[ \begin{aligned}
\Theta_1(z) &= \frac{1/\gamma^2}{1/\gamma - 1 - zm(z)} - \frac1\gamma \\
& = \frac1 \gamma \left(\frac{1}{1 - \gamma(1+zm(z)) } - 1\right)\\
& = \frac1\gamma \left( -\frac{1}{z\nu(z)} - 1 \right).
\end{aligned} \]


Also, from lemma 3 in \cite{ledoit2011eigenvectors} we have \[ \Theta_{k+1}(z) = \left[z\Theta_k(z) + \int s^kdH \right]\times \left[1+\gamma \Theta_1(z)\right]. \] These are the preliminary definitions and results required to prove the following theorem.

\begin{theorem}
Assume the prior $P_{\beta, \delta}$ for $\beta$ and $\delta$ with the following moments: \[E(\beta) = E(\delta) = 0, \quad E(\beta\beta^T) = \frac{r_\beta^2}p I, \quad E(\delta\delta^T) = \frac{r_\delta^2}p I, \quad E(\beta\delta^T) = \frac{r_{\beta, \delta}}p I \] 
\[  
R(\hat \beta)  \to \begin{cases} \frac{r_\beta^2}{\gamma \nu(0)} + \frac{r_\delta^2\pi}{\gamma\nu(0)}\left(\gamma \nu(0)\int s dH - 1\right)  \left[   (1-\pi)\gamma \nu(0)\int s dH   +   \pi   \right]
 & \text{for } \gamma > 1\\
 \quad  + \sigma^2 \left(\frac{\nu'(0)}{\nu^2(0)}-1\right)\\
 \frac{r_\delta^2\pi}{\gamma(1-\gamma)} \int sdH \big[ \gamma^2 + \pi\gamma (1-2\gamma) \big] + \sigma^2 \frac\gamma{1-\gamma}
  & \text{for } \gamma < 1
 \end{cases} 
\] 

\end{theorem}


\begin{proof}
	The estimation error 
	\[
	\begin{aligned}
	\hat \beta - \beta_0 & =  (X^TX)^{+}X^T(X\beta_0 + \begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + \eps) - \beta_0\\
	& = \big((X^TX)^{+}X^TX - I\big)\beta_0   + (X^TX)^{+}X^T\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + (X^TX)^{+}X^T\eps\\
	& = \big(X^T(XX^T)^{-1}X - I\big)\beta_0   + X^T(XX^T)^{-1}\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + (X^TX)^{+}X^T\eps
	\end{aligned}
	\]
Let us define $ \Pi = (X^TX)^+ X^TX .$	The MSPE is 
	\[
	\begin{aligned}
	R(\hat\beta) & = E\big[  (\hat \beta - \beta_0)^T \Sigma (\hat \beta - \beta_0) \big] \\
	& = E \big[  \beta_0^T (I - \Pi ) \Sigma (I-\Pi)\beta_0  \big] + E\big[ \eps^T X (X^TX)^{+} \Sigma (X^TX)^{+} X^T \eps  \big] \\
	& \quad + E\big[  \delta^T X_1^TX_1 (X^TX)^{+} \Sigma (X^TX)^{+} X_1^T X_1 \delta  \big]\\
	& \quad - 2 E \Big[ \beta_0^T (I - \Pi ) \Sigma (X^TX)^{+}X^T\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta  \Big]\\
	& \quad = B(\hat \beta) + V(\hat\beta) + B_2(\hat \beta) - 2C(\hat \beta)
	\end{aligned}
	\]
	\paragraph{Calculation of $B(\hat \beta)$}
	
	If $\gamma >1$
	\[
	\begin{aligned}
	(I - \Pi ) \Sigma (X^TX)^{+}X^T & = (I - X^T (XX^T)^{-1}X ) \Sigma X^T(XX^T)^{-1}
	\end{aligned}
	\]
	
	
	\[
	\begin{aligned}
	B(\hat \beta ) & = E\big[ \beta_0 ^T (I - \Pi) \Sigma (I - \Pi) \beta_0 \big]\\
	& = \frac{\|\beta_0 \|_2^2}{p} E\big[\text{Tr} \big((I-\Pi)\Sigma (I-\Pi)\big) \Big] \\
	& = r_\beta^2 E\Big[\frac1p\text{Tr} \big((I - \Pi)\Sigma\big)  \Big]\\
	& = \frac{r_\beta^2}{\gamma \nu(0-)}
	\end{aligned}
	\]
	since
	\[
	\begin{aligned}
	\frac1p\text{Tr} \big((I - \Pi)\Sigma\big) & = \lim_{z\to 0+} \frac1p\text{Tr} \big[(I - (X^TX+nzI)^{-1}(X^TX))\Sigma\big]\\
	& = \lim_{z\to 0+}  \frac{nz}{p} \text{Tr} \big[ (X^TX+nzI)^{-1}\Sigma\big]\\
	& = \lim_{z\to 0+}  \frac{z}{p} \text{Tr} \big[ (X^TX/n+zI)^{-1}\Sigma\big]\\
	& = \lim_{z\to 0+}  \frac{z}{p} \text{Tr} \big[ (\hat \Sigma+zI)^{-1}\Sigma\big]\\
	& \to \lim_{z\to 0+} z \Theta_1(-z)\\
	& = \lim_{z\to 0+} z \frac1 \gamma \left(-1 + \frac{1}{z\nu(-z)}\right)\\
	& = \frac{1}{\gamma \nu(0-)}
	\end{aligned}
	\]
	If $\gamma < 1$ we have $B(\hat \beta )  = 0.$
	
	
	\paragraph{Calculation of $V(\hat \beta)$}
	If $\gamma >1$ then 
	\[
	\begin{aligned}
	 V(\hat \beta)& = E\big[ \eps^T X (X^TX)^{+} \Sigma (X^TX)^{+} X^T \eps  \big] \\
	 & = \sigma^2 E\Big[\text{Tr}\big\{  (X^TX)^{+} \Sigma (X^TX)^{+} X^T X  \big\}\Big]\\
	&  = \sigma^2 \lim_{z\to 0+} E\Big[\text{Tr}\big\{  (X^TX+nzI)^{-1} \Sigma (X^TX+nzI)^{-1} X^T X  \big\}\Big]\\
	&  = \sigma^2\frac1 n \lim_{z\to 0+} E\Big[\text{Tr}\big\{  (X^TX/n+zI)^{-1} \Sigma (X^TX/n+zI)^{-1} (X^T X/n)  \big\}\Big]\\
	&  = \sigma^2\gamma \lim_{z\to 0+}\frac1 p E\Big[\text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma (\hat \Sigma+zI)^{-1} \hat \Sigma  \big\}\Big]\\
	& = \sigma^2 \left( \frac{\nu'(0)}{\nu^2(0)} -1 \right)
	\end{aligned}
	\]
	since, 
	\[
	\begin{aligned}
	& \lim_{z\to 0+}\frac1 p \text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma (\hat \Sigma+zI)^{-1} \Sigma  \big\}\\
	& \quad = \lim_{z\to 0+}\left[\frac1 p \text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma  \big\} - z \frac 1p\text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma (\hat \Sigma+zI)^{-1}   \big\}\right]\\
	& \quad = \lim_{z\to 0+}\left[\frac1 p \text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma  \big\} - z \frac 1p\text{Tr}\big\{  (\hat \Sigma+zI)^{-2} \Sigma    \big\}\right]\\
	& \quad = \lim_{z\to 0+}\left[\frac1 p \text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma  \big\} + z \frac{d}{dz}\left(\frac 1p\text{Tr}\big\{  (\hat \Sigma+zI)^{-1} \Sigma    \big\}\right)\right]\\
	& \quad \to \lim_{z\to 0+} \big( \Theta_1(-z) + z \Theta_1'(-z) \big)\\
	& \quad = \lim_{z\to 0+} \big( z\Theta_1(-z)  \big)'\\
	& \quad = \lim_{z\to 0+}\frac 1 \gamma \big( -z + \frac 1{\nu(-z)}  \big)'\\
	& \quad = \lim_{z\to 0+} \frac{1}{\gamma} \left(-1 + \frac{\nu'(-z)}{\nu^2(-z)} \right)\\
	& \quad = \frac{1}{\gamma} \left(-1 + \frac{\nu'(0)}{\nu^2(0)} \right)
	\end{aligned}
	\]
	
	If $\gamma < 1$ then \[
	\begin{aligned}
	V(\hat \beta)
	 & = \sigma^2 E\Big[\text{Tr}\big\{  (X^TX)^{+} \Sigma (X^TX)^{+} X^T X  \big\}\Big]\\
	 & = \sigma^2 E\Big[\text{Tr}\big\{  (X^TX)^{-1} \Sigma   \big\}\Big]\\
	 & = \sigma^2 E\Big[\text{Tr}\big\{  \big(\Sigma^{-1/2}X^TX\Sigma^{-1/2}\big)^{-1}   \big\}\Big]\\
	 & = \sigma^2 \frac1n E\Big[\text{Tr}\big\{  \big(Z^TZ/n\big)^{-1}   \big\}\Big]\\
	 & = \sigma^2 \gamma \frac1p  E\Big[\text{Tr}\big\{  \big(Z^TZ/n\big)^{-1}   \big\}\Big]\\
	 & = \sigma^2 \frac\gamma{1-\gamma}
	\end{aligned}
	\]
	\paragraph{\underline{Calculation of $B_2(\hat \beta)$}}
	For $\gamma>1$
	\[
	\begin{aligned}
	B_2(\hat \beta) & = E\big[  \delta^T X_1^TX_1 (X^TX)^{+} \Sigma (X^TX)^{+} X_1^T X_1 \delta  \big]\\
	& = \frac{r_\delta^2}{p} E\big[ \text{Tr} \big\{  X_1^TX_1 (X^TX)^{+} \Sigma (X^TX)^{+} X_1^T X_1 \big\}  \big]\\
	& = \frac{r_\delta^2}{p} E\left[ \sum_{i,j = 1}^{n_1} \text{Tr} \big\{  x_ix_i^T  (X^TX)^{+} \Sigma (X^TX)^{+} x_j x_j^T \big\}  \right]\\
	& = n_1\frac{r_\delta^2}{p} E\left[ x_1^T  x_1x_1^T  (X^TX)^{+} \Sigma (X^TX)^{+} x_1  \right]\\
	& \quad  + n_1(n_1 - 1)\frac{r_\delta^2}{p} E\left[ x_1^T  x_2x_1^T  (X^TX)^{+} \Sigma (X^TX)^{+} x_2  \right]\\
	& = \frac{r_\delta^2}{p} \big[n_1 D_1 + n_1(n_1-1)D_2 \big]
	\end{aligned}
	\]
	
	
	\[
	\begin{aligned}
	D_1 & =  (x_1^T x_1)  x_1^T  (X^TX)^{+} \Sigma (X^TX)^{+} x_1\\
	&  = \lim_{z\to 0+} x_1^T x_1  x_1^T  (X^TX + (n-1)zI)^{-1} \Sigma (X^TX + (n-1)zI)^{-1} x_1 \\
	&  = \lim_{z\to 0+} (x_1^T x_1)  x_1^T  ( x_1x_1^T +  X_{-1}^TX_{-1} + (n-1)zI)^{-1} \Sigma (x_1x_1^T + X_{-1}^TX_{-1} + (n-1)zI)^{-1} x_1\\
	&  = \lim_{z\to 0+}(x_1^T x_1)   x_1^T  \left(A^{-1} - \frac{A^{-1} x_1 x_1 ^T A^{-1}}{1 + x_1^TA^{-1}x_1}\right)  \Sigma \left(A^{-1} - \frac{A^{-1} x_1 x_1 ^T A^{-1}}{1 + x_1^TA^{-1}x_1}\right) x_1,\quad \text{where } A = X_{-1}^T X_{-1} + (n-1)zI, \\
	&  = \lim_{z\to 0+} \frac{(x_1^T x_1) x_1^T A^{-1}\Sigma A^{-1}x_1}{(1+x_1^TA^{-1}x_1)^2}\\
	&  = \lim_{z\to 0+} \frac{(x_1^T x_1) \frac 1 {(n-1)^2} x_1^T (\hat \Sigma' + zI )^{-1}\Sigma (\hat \Sigma' + zI)^{-1}x_1}{\left(1+\frac1 {n-1}x_1^T(\hat \Sigma' + zI )^{-1}x_1\right)^2}\\
	&  = \lim_{z\to 0+} \frac{\gamma^2(\frac1p x_1^T x_1) \frac 1 {p} x_1^T z^2 (\hat \Sigma' + zI )^{-1}\Sigma (\hat \Sigma' + zI)^{-1}x_1}{\left(z+\gamma\frac1 {p}x_1^Tz(\hat \Sigma' + zI )^{-1}x_1\right)^2}
	\end{aligned}
	\] where $ \hat \Sigma' = X_{-1}^TX_{-1}/(n-1). $
	Using lemma \ref{lemma:conv-parts} we get \[ 
	\begin{aligned}
	D_1 & = \lim_{z\to 0+} \frac{\gamma^2(\frac1p x_1^T x_1) \frac 1 {p} x_1^T z^2 (\hat \Sigma' + zI )^{-1}\Sigma (\hat \Sigma' + zI)^{-1}x_1}{\left(z+\gamma\frac1 {p}x_1^Tz(\hat \Sigma' + zI )^{-1}x_1\right)^2} \\
	& \to \lim_{z\to 0+} \frac{\left(\int s dH\right)z^2\gamma^2 \big(- \Theta_2(-z)\big)'}{\big(z+\gamma z\Theta_1(-z)\big)^2}\\
	& = \lim_{z\to 0+} \frac{\left(\int s dH\right)z^2\gamma^2 \frac{d}{dz}\left[\left( z\Theta_1(-z) - \int s dH\right)\left(1 + \gamma\Theta_1(-z)\right)\right]}{\big(z+\gamma z\Theta_1(-z)\big)^2}\\
	& = \lim_{z\to 0+} \frac{\gamma\left(\int s dH\right)z^2 \frac{d}{dz}\left[\left( \gamma z\Theta_1(-z) - \gamma \int s dH\right)\left(1  + \gamma\Theta_1(-z)\right)\right]}{\gamma\big(z+\gamma z\Theta_1(-z)\big)^2}\\
	& = \lim_{z\to 0+} \frac{\gamma\left(\int s dH\right)z^2 \frac{d}{dz}\left[\left( -z + \frac 1{\nu(-z)} - \gamma \int s dH\right)\left( \frac{1}{ z \nu(-z)} \right)\right]}{\big(\frac1{\nu(-z)}\big)^2}\\
	& = \lim_{z\to 0+} \gamma \left(\int s dH\right)z^2 \nu^2 (-z) \left[\left( -1 + \frac {\nu'(-z)}{\nu^2(-z)} \right)\left( \frac{1}{ z \nu(-z)}  \right)\right.\\
	& \quad\quad\quad   + \left. \left( -z + \frac 1{\nu(-z)} - \gamma \int s dH\right)\left(- \frac{1}{ z^2 \nu(-z)} +\frac {\nu'(-z)}{ z\nu^2(-z)} \right) \right]\\
	& = \gamma\left(\int s dH\right) \nu^2(0) \left(\gamma \int s dH  - \frac1 {\nu(0)}\right)\frac1{ \nu(0)}\\
	& = \gamma \left(\int s dH\right)  \left(\gamma \nu(0)\int s dH - 1\right)
	\end{aligned} \]


	We also notice
	\[ \text{Tr} \big\{  x_1x_1^T (X^TX)^{+} \Sigma (X^TX)^{+} (X^T X) \big\} = D_1 + (n-1)D_2. \] We shall try to compute the in probability limit of the term $ \text{Tr} \big\{  x_1x_1^T (X^TX)^{+} \Sigma (X^TX)^{+} (X^T X) \big\} $ which shall provide the same for $ D_2. $
	
	Note that
	 \[ \begin{aligned}
	& \text{Tr} \big\{  x_1x_1^T (X^TX)^{+} \Sigma (X^TX)^{+} (X^T X) \big\}\\
	& \quad = \lim_{z\to 0+} \text{Tr} \big\{  x_1x_1^T (X^TX + (n-1)zI)^{-1} \Sigma (X^TX + (n-1)zI)^{-1} (X^T X) \big\}\\
	& \quad = \lim_{z\to 0+}x_1^T (X^TX + (n-1)zI)^{-1} \Sigma (X^TX + (n-1)zI)^{-1} (X^T X) x_1\\
	& \quad = \lim_{z\to 0+}\left[x_1^T (X^TX + (n-1)zI)^{-1} \Sigma  x_1\right.\\
	& \quad \quad \quad\left. - (n-1)zx_1^T (X^TX + (n-1)zI)^{-1} \Sigma (X^TX + (n-1)zI)^{-1}  x_1 \right]
	\end{aligned}\]
	Now, \[ \begin{aligned}
	& \lim_{z\to 0+} x_1^T (X^TX + (n-1)zI)^{-1} \Sigma  x_1\\
	& \quad = \lim_{z\to 0+} x_1^T \big(x_1 x_1^T + X_{-1}^TX_{-1} + (n-1)zI\big)^{-1} \Sigma  x_1\\
	& \quad = \lim_{z\to 0+} x_1^T \left(\big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1}\right.\\
	&\quad \quad \quad\left. -\frac{ \big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1}x_1x_1^T\big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1}}{1 + x_1^T\big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1}x_1}\right) \Sigma  x_1\\
	& \quad = \lim_{z\to 0+}\frac{x_1^T\big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1}\Sigma x_1}{1+ x_1^T\big( X_{-1}^TX_{-1} + (n-1)zI\big)^{-1} \Sigma  x_1}\\
	& \quad = \lim_{z\to 0+}\frac{\frac1{n-1}x_1^T\big( \hat \Sigma' + zI\big)^{-1}\Sigma x_1}{1+ \frac1{n-1}x_1^T\big( \hat \Sigma' + zI\big)^{-1} \Sigma  x_1}\\
	& \quad = \lim_{z\to 0+}\frac{\gamma z\frac1{p}x_1^T\big( \hat \Sigma' + zI\big)^{-1}\Sigma x_1}{z+ \gamma z\frac1{p}x_1^T\big( \hat \Sigma' + zI\big)^{-1} \Sigma  x_1}\\
	& \quad \to \lim_{z\to 0+}\frac{\gamma z\Theta_2(-z)}{z+ \gamma z\Theta_1(-z)}\\
	& \quad = \lim_{z\to 0+}\frac{\gamma z\left(\int s dH - z\Theta_1(-z)\right)\left(1+\gamma \Theta_1(z)\right)}{\frac1{\nu(-z)}}\\
	& \quad = \lim_{z\to 0+}\nu(-z) \left(\gamma \int s dH - \gamma z\Theta_1(-z)\right)\left(z+z\gamma \Theta_1(z)\right)\\
	& \quad = \lim_{z\to 0+}\nu(-z) \left(\gamma \int s dH - \frac1 {\nu(-z)} + z\right)\left( \frac{1}{ \nu(-z)} \right)\\
	& \quad \to \nu(0) \left(\gamma \int s dH - \frac1 {\nu(0)} \right)\frac{1}{ \nu(0)}\\
	& \quad = \frac{1}{ \nu(0)} \left(\gamma \int s dH \nu(0)-1 \right)
	\end{aligned} \]
	
	and \[ \begin{aligned}
	& \lim_{z\to 0+} (n-1)zx_1^T (X^TX + (n-1)zI)^{-1} \Sigma (X^TX + (n-1)zI)^{-1}  x_1\\
	& \quad = \lim_{z\to 0+} \frac1{n-1}zx_1^T (\hat\Sigma + zI)^{-1} \Sigma (\hat\Sigma + zI)^{-1}  x_1\\
	& \quad = 0
	\end{aligned} \]
	where the limit is zero because $  \frac1{n-1}x_1^T (\hat\Sigma + zI)^{-1} \Sigma (\hat\Sigma + zI)^{-1}  x_1 $ converges to a finite limit. 
	
	Hence, we get \[ 
	\begin{aligned}
	(n-1)D_2 &= \frac{1}{ \nu(0)} \left(\gamma \int s dH \nu(0)-1 \right) - \gamma \left(\int s dH\right)  \left(\gamma \nu(0)\int s dH - 1\right)\\
	& = -\frac{1}{ \nu(0)} \left(\gamma \nu(0)\int s dH - 1\right)^2
	\end{aligned} \]
	Finally, we get \[ \begin{aligned}
	B_2(\hat \beta) 
	& = \frac{r_\delta^2}{p} \big[n_1 D_1 + n_1(n_1-1)D_2 \big]\\
	& \asymp r_\delta^2 \left[\frac\pi\gamma  D_1 + \frac{\pi^2}\gamma (n-1) D_2 \right]\\
	& \asymp r_\delta^2 \left[  \frac\pi\gamma \gamma \left(\int s dH\right)  \left(\gamma \nu(0)\int s dH - 1\right) - \frac{\pi^2} \gamma \frac{1}{ \nu(0)} \left(\gamma \nu(0)\int s dH - 1\right)^2  \right]\\
	& = \frac{r_\delta^2\pi}{\gamma\nu(0)}\left(\gamma \nu(0)\int s dH - 1\right)  \left[   \left(\gamma \nu(0)\int s dH\right)   - \pi  \left( \gamma\nu(0)\int s dH - 1\right)  \right]\\
	& = \frac{r_\delta^2\pi}{\gamma\nu(0)}\left(\gamma \nu(0)\int s dH - 1\right)  \left[   (1-\pi)\gamma \nu(0)\int s dH   +   \pi   \right]
	\end{aligned} \]
\end{proof}


\begin{lemma}[\cite{ledoit2011eigenvectors}, lemma 1]
	\label{lemma:conv-quadratic-exp}
	Let $Y = (y_1, \dots, y_N)$ be a random vector with \iid\ entries satisfying:
	\[ E y_1 = 0, \quad E y_1^2 = 1, \quad Ey_1^{12} \le B  \] where the constant $ B $ doesn't depend on $ N .$ Let also $ A $ be a $ N \times N $ matrix. Then there exists a constant $ K>0 $ independent of $ Y, A, N $ such that: \[
	E\left|  Y^T AY - \text{Tr} (A) \right|^6 \le K\|A\|_{\text{op}} N^3.
	\] 
	Furthermore, if $ \|A\|_{\text{op}} N^3 \to 0  $ as $ N\to \infty $ then \[
	Y^T AY -  \text{Tr} (A)\to 0  \text{ in probability.}
	\] 
\end{lemma}


\begin{lemma}
	\label{lemma:conv-parts}
	The following in probability convergence holds: 
	\begin{enumerate}
		\item $ \frac1 p x_1^Tx_1 \to \int s dH, $
		\item $ \frac1 {p}x_1^Tz(\hat \Sigma + zI )^{-1}\Sigma^j x_1 \to z \Theta_{j+1}(-z),  $
		\item $ \frac 1 {p} x_1^T z^2 (\hat \Sigma + zI )^{-1}\Sigma (\hat \Sigma + zI)^{-1}x_1 \to z^2 (-\Theta_2(-z))' $
	\end{enumerate}
	
\end{lemma}

\begin{proof}
	We shall use \ref{lemma:conv-parts} repeatedly. 
	
	
	\textbf{(1)} Note that $ \frac1 p x_1^Tx_1 = z_1^T (\Sigma/p) z_1. $ Here $ \|\Sigma/p\|_{\text{op}} p^3 = \sigma_{\text{max}} \frac{\sigma_{\text{max}}^6}{p^3} \to 0. $ Hence, \[ 
	\frac1 p x_1^Tx_1  - \int s dH = \frac1 p x_1^Tx_1 -   \text{Tr} (\Sigma/p) + \frac1p  \text{Tr} (\Sigma) - \int s dH \to 0.
	\]
	
	\textbf{(2)} Here $  \frac1 {p}x_1^Tz(\hat \Sigma + zI )^{-1}\Sigma^j x_1 =  z_1^T\left(\frac{\Sigma ^{1/2}(z\hat \Sigma + I )^{-1}\Sigma ^{1/2+j}}{p}\right)z_1 $ and \[ 
	\begin{aligned}
	\left\|\frac{\Sigma ^{1/2}(\hat \Sigma/z + I )^{-1}\Sigma ^{1/2+j}}{p}\right\|_{\text{op}} & \le \frac1p \|\Sigma^{1/2}\|_{\text{op}}  \|(\hat \Sigma/z + I )^{-1}\|_{\text{op}} \|\Sigma^{1/2+j}\|_{\text{op}} \\
	&\le  \frac{\sigma_{\text{max}}}{p}^{j+1}
	\end{aligned} \] This implies \[	\left\|\frac{\Sigma ^{1/2}(\hat \Sigma/z + I )^{-1}\Sigma ^{1/2+j}}{p}\right\|_{\text{op}}^{6+6j} p^3 \to 0,   \] and we get \[ 
	\frac1 {p}x_1^Tz(\hat \Sigma + zI )^{-1}\Sigma^jx_1 - \text{Tr} \left(\frac{\Sigma ^{1/2}z(\hat \Sigma + zI )^{-1}\Sigma ^{1/2+j}}{p}\right) \to 0
	\]in probability. Since, \[ \text{Tr} \left(\frac{\Sigma ^{1/2}z(\hat \Sigma + zI )^{-1}\Sigma ^{1/2+j}}{p}\right) \to z \Theta_{j+1}(-z) \] in probability, we have the result. 
	
	\textbf{(3)} Note that \[ \begin{aligned}
	& \frac 1 {p} x_1^T z^2 (\hat \Sigma + zI )^{-1}\Sigma (\hat \Sigma + zI)^{-1}x_1\\
	&\quad  = \frac 1 {p} z_1^T \Sigma^{1/2} z^2 \Sigma^{-1/2} \big(\Sigma^{-1/2}\hat \Sigma \Sigma^{-1/2} + z\Sigma^{-1} \big)^{-1}\Sigma^{-1/2}\Sigma\Sigma^{-1/2} \big(\Sigma^{-1/2}\hat \Sigma\Sigma^{-1/2} + z\Sigma^{-1}\big)^{-1}\Sigma^{-1/2}\Sigma^{1/2}z_1\\
	& \quad = \frac 1 {p} z_1^T  z^2  \big(\Sigma^{-1/2}\hat \Sigma \Sigma^{-1/2} + z\Sigma^{-1} \big)^{-2} z_1\\
	& \quad =  z_1^T \left(\frac{   \Sigma\big(\hat \Sigma/z  + I \big)^{-2}\Sigma}{p}\right) z_1
	\end{aligned} \] and \[ \begin{aligned}
	\left\|\frac{   \Sigma\big(\hat \Sigma/z  + I \big)^{-2}\Sigma}{p} \right\|_{\text{op}} \le \frac1 p \sigma_{\text{max}}^2 .
	\end{aligned} \] This implies \[ \left\|\frac{   \Sigma\big(\hat \Sigma/z  + I \big)^{-2}\Sigma}{p} \right\|_{\text{op}}^6 p^3 \le \frac 1{p^3} \sigma_{\text{max}}^{12}\to 0 \] which gives us \[ \frac 1 {p} x_1^T z^2 (\hat \Sigma + zI )^{-1}\Sigma (\hat \Sigma + zI)^{-1}x_1 - \text{Tr}\left(\frac{   \Sigma\big(\hat \Sigma/z  + I \big)^{-2}\Sigma}{p}\right) \to 0 \] in probability. Since, \[ \begin{aligned}
	\text{Tr}\left(\frac{   \Sigma^{1/2}\big(\hat \Sigma/z  + I \big)^{-2}\Sigma^{1/2}}{p}\right) &= \frac{z^2}{p}\text{Tr}\left(   \big(\hat \Sigma/z  + I \big)^{-2}\Sigma^2\right)\\
	& = - z^2\frac{d}{dz}\left(\frac1p\text{Tr}\left(   \big(\hat \Sigma/z  + I \big)^{-1}\Sigma^2\right)  \right)\\
	& \to - z^2 \frac{d}{dz} \big(\Theta_2(-z)\big)
	\end{aligned} \] in probability, we have the result.
	
	
	For $\gamma<1$ we note that 
	
	\[m(0) = \int\frac1s dG_{X^TX/n} (s), \quad m'(0) =\int\frac1{s^2} dG_{X^TX/n} (s)  \] are finite quantities. Hence from  \[ \begin{aligned}
\Theta_1(z) &= \frac{1/\gamma^2}{1/\gamma - 1 - zm(z)} - \frac1\gamma \\
& = \frac1 \gamma \left(\frac{1}{1 - \gamma(1+zm(z)) } - 1\right)
\end{aligned} \] we get \[ \Theta_1(-z) = \frac1{1-\gamma} \] as $z \to 0+.$

\[
	\begin{aligned}
	D_1 & =  (x_1^T x_1)  x_1^T  (X^TX)^{-1} \Sigma (X^TX)^{-1} x_1\\
    &  = (x_1^T x_1)   x_1^T  \left(A^{-1} - \frac{A^{-1} x_1 x_1 ^T A^{-1}}{1 + x_1^TA^{-1}x_1}\right)  \Sigma \left(A^{-1} - \frac{A^{-1} x_1 x_1 ^T A^{-1}}{1 + x_1^TA^{-1}x_1}\right) x_1,\\
	&\quad\quad \text{where } A = X_{-1}^T X_{-1}, \\
	&  =  \frac{(x_1^T x_1) x_1^T A^{-1}\Sigma A^{-1}x_1}{(1+x_1^TA^{-1}x_1)^2}\\
	&  =  \frac{(x_1^T x_1) \frac 1 {(n-1)^2} x_1^T (\hat \Sigma'  )^{-1}\Sigma (\hat \Sigma' )^{-1}x_1}{\left(1+\frac1 {n-1}x_1^T(\hat \Sigma'  )^{-1}x_1\right)^2}\\
	&  =  \frac{\gamma^2(\frac1p x_1^T x_1) \frac 1 {p} x_1^T  (\hat \Sigma' )^{-1}\Sigma (\hat \Sigma' )^{-1}x_1}{\left(1+\gamma\frac1 {p}x_1^T(\hat \Sigma' )^{-1}x_1\right)^2}\\
	& \to \frac{\gamma^2\left(\frac1 p \text{Tr}(\Sigma)\right)\left( \frac 1 {p} \text{Tr}\big(\Sigma  (\hat \Sigma' )^{-1}\Sigma (\hat \Sigma' )^{-1}\big)\right)}{\left(1+\gamma\frac1 {p}\text{Tr}\big(\Sigma\hat (\Sigma')^{-1} \big)\right)^2}
	\end{aligned}
	\]

Here $\frac1p\text{Tr}(\Sigma) \to \int sdH $, \[
\begin{aligned}
\frac1 {p}\text{Tr}\big(\Sigma\hat (\Sigma')^{-1} \big) & = \frac1 {p}\text{Tr}\big(\hat (\Sigma^{-1/2}\Sigma'\Sigma^{-1/2})^{-1} \big)\\
& = m_{I}(0) = \frac1{1-\gamma}
\end{aligned}
\] and 
\[
\begin{aligned}
\frac 1 {p} \text{Tr}\big(\Sigma  (\hat \Sigma' )^{-1}\Sigma (\hat \Sigma' )^{-1}\big) & = \frac1 {p}\text{Tr}\big( (\Sigma^{-1/2}\Sigma'\Sigma^{-1/2})^{-2} \big)\\
& = m_{I}'(0) = \frac1{(1-\gamma)^3}
\end{aligned}
\] where $m_I$ is the Stieltzes transform with $\Sigma = I.$ 
Hence, \[
\begin{aligned}
D_1 & \to \frac{\gamma^2\int sdH\frac1{(1-\gamma)^3}}{\left(1+\frac\gamma{(1-\gamma)}\right)^2}\\
& = \frac{\gamma^2}{1-\gamma}\int sdH
\end{aligned}
\] Furthermore, 
\[
\begin{aligned}
& D_1 + (n-1)D_2 \\
& \quad = \gamma\frac1p \big(nD_1 + n(n-1)D_2\big) \\
&\quad = \gamma\frac1p \text{Tr} \big\{  X^TX (X^TX)^{-1} \Sigma (X^TX)^{-1} (X^T X) \big\}\\
& \quad =\gamma \frac{1}{p}\text{Tr}(\Sigma)\\
& \quad \to \gamma\int sdH
\end{aligned}
\]
Hence \[ (n-1)D_2 = \gamma\int sdH - \frac{\gamma^2}{1-\gamma}\int sdH = \gamma\left(\frac{1-2\gamma}{1-\gamma}\right)\int sdH.\]

Hence, \[
\begin{aligned}
B_2(\hat\beta) &  = \frac{r_\delta^2}{p} \big[n_1 D_1 + n_1(n_1-1)D_2 \big]\\
& \asymp r_\delta^2\frac\pi\gamma \left(\frac{\gamma^2}{1-\gamma}\int sdH + \pi (n-1)D_2 \right)\\
& \asymp r_\delta^2\frac\pi\gamma \left(\frac{\gamma^2}{1-\gamma}\int sdH + \pi \gamma\left(\frac{1-2\gamma}{1-\gamma}\right)\int sdH \right)\\
& = \frac{r_\delta^2\pi}{\gamma(1-\gamma)} \int sdH \big[ \gamma^2 + \pi\gamma (1-2\gamma) \big]
\end{aligned}
\]

\paragraph{Calculation of $C(\hat \beta)$}
If $\gamma>1$ then 
\[
\begin{aligned}
& E \Big[ \beta_0^T (I - \Pi ) \Sigma (X^TX)^{+}X^T\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta  \Big] \\
&\quad = \frac{n_1}n E \Big[ \beta_0^T (I - \Pi ) \Sigma (X^TX)^{+}X^TX\delta  \Big]\\
&\quad = \pi r_{\beta, \delta} E \left[\text{Tr}\Big[  (I - \Pi ) \Sigma \Pi  \Big]\right]\\
&\quad =0
\end{aligned}
\]
If $\gamma < 1$ then $\Pi = I$ and hence $C(\hat \beta) = 0.$
\end{proof}


==> rebuttal.tex <==
Reviewer jgBW:

Replacing risk with model output in the fairness definition of demographic parity and equalised odds is assuming that the loss function used in learning is the same as that for fairness consideration. The advantage of enforcing independence with model output is that it will ensure independence with any fairness loss function. For many reasons such as ease of optimization (use of surrogate loss) or application context, the two loss functions can be different. This critical assumption should be stated.



The target for comparison in the unbiased data is assumed to be the unconstrained Bayes optimal model. I disagree with the claim that assumption 3 is implicitly assumed in many previous works, lines 229-235. The cited works are not suggesting to just use the unconstrained Bayes classifier on representative data. The classifier for unbiased data can be trained with fairness constraints too if suitable for the application context.


Label bias described in Example 4.2 differs from the subpopulation shift assumption. It is usually defined as an invariant distribution of outcome given some or all covariates, whereas the label bias and the resulting risk profile is additionally conditioning on the outcome. Please define subpopulation shifts in the Problem setup to avoid any confusion.



Is the risk profile in 4.2 defined with respect to biased distribution P tilde?


Are the conditions for checking improvement in the theorems testable? What data does it require?


How to interpret the threshold on P* in Theorem 3.2 which is used to check whether FRM improves?


In Theorem 4.3 assumptions, which risk set or profile is used, 3.1 or 4.2?


Please clarify how the results can be used to better evaluate and design fair classifiers.





Reviewer 3vrA:





Reviewer M7Vx:


 One should be careful with interpreting results of this paper as the paper assumes the assumption in equation (3.3). This is assumption 2 under Theorem 3.2 and 4.3. It means that this paper does not consider an entire distribution shift from the train domain to the target domain and restricts its attention to subpopulation shift. Hence, one should be cautious about making general statements based on this paper. Perhaps, a discussion about this can help the general reader more.
 
 
 
 Contribution number 3 in Introduction: Line 36, please complete the sentence.
 
 
 
 
 Reviewer VZHD:
 


 It seems that assumption (3.3) is fairly limiting. For example, this assumption rules out the setting of label-bias as defined by [1] and thus. In addition, I looked at the paper in reference [16] (line 92), and I have the impression that (3.3) is an additional assumption imposed on the subpopulation shifts setting, rather than being “(slightly) less restrictive”.
 
 
 That said, it is unclear to me why the bounds per se, in their current form, should be of interest, or at least I do not think that the result in theorem 3.2 was properly discussed. We should probably interested in understanding by how much performance will change, although I am not sure this is analytically possible.
 
 
 Suggestions: (i) move related work up and clearly explain how this work fits into the existing literature, (ii) clearly define all notation, (iii) improve the explanations of the results, (iv) add an organization paragraph in the introduction.



==> ridgeless-setup-YK.tex <==
The learner fits a linear model $f(x) \triangleq \beta^Tx$ to the training data, where $\beta\in\reals^d$ is a vector of regression coefficients. The learner's choice is motivated by two considerations:
\begin{enumerate}
\item it is well-specified for the majority group. If the learner simply picks a model that performs well on the majority group, then the linear model is a good choice.
\item it does not use the sensitive attribute (group membership). Although group membership is observed in the training data, it is unobserved at test time in most applications, so models that use group membership are not useful in such applications.
\end{enumerate}
We note that although the linear model is well-specified for each group, it is \emph{misspecified} for the mixture of two groups. The learner fits a linear model to the training data in one of three ways: empirical risk minimization, reweighing, and subsampling.

\subsection{Empirical risk minimization (ERM)} 

The most common way of fitting a linear model is ordinary least squares (OLS):
\[\textstyle
\hbeta_{\OLS} \in \argmin_{\beta\in\reals^d}\frac1n\sum_{i=1}^n\frac12(y_i - \beta^Tx_i)^2 = \argmin_{\beta\in\reals^d}\frac{1}{2n}\|y - X\beta\|_2^2,
\]
where the rows of $X\in\reals^{n\times d}$ are the $x_i$'s and the entries of $y\in\reals^n$ are the $y_i$'s. We note that ERM does not use the sensitive attribute (even during training), so it is suitable for problems in which the training data does not include the sensitive attribute.

In the overparameterized case ($n < d$), $\hbeta_{\OLS}$ is not well-defined because there are many linear models that can interpolate the training data. In this case, we consider the minimum $\ell_2$ norm (min-norm) linear model with zero training error:
\[\textstyle
\hbeta_{\min} \in \argmin\{\|\beta\|_2\mid y = X\beta\} = (X^TX)^\dagger X^Ty.
\]
where $(X^TX)^\dagger$ denotes the Moore-Penrose pseudoinverse of $X^TX$. The min-norm least squares estimator is also known as the ridgeless least squares estimator because $\hbeta_{\min} = \lim_{\lambda\searrow 0}\hbeta_\lambda$, where
\[\textstyle
\hbeta_\lambda \in \argmin_{\beta\in\reals^d}\frac1n\|y-X\beta\|_2^2 + \lambda\|\beta\|_2^2.
\]
We note that if $X$ has full column rank (\ie\ $X^TX$ is non-singular), then $\hbeta_{\min}$ is equivalent to $\hbeta_{\OLS}$. 

\subsection{Reweighted empirical risk minimization} 

It is known that models trained by ERM may perform poorly on minority groups \cite{sagawa2019Distributionally}. To encourage the model to perform better on minority groups during training, the learner may upweigh (the loss on) training samples from the minority group:
\[
\tbeta_{\ERM} \in \argmin_{\beta\in\reals^d}\tilde{R}(\beta),
\]
where
\[
\tilde{R}(\beta) \triangleq \frac1n\left\{\begin{aligned}&\textstyle\frac{1}{\pi}\sum_{i=1}^n\frac12(y_i - \beta^Tx_i)^2\ones\{g_i = 0\} \\
&\textstyle+\frac{1}{1-\pi}\sum_{i=1}^n\frac12(y_i - \beta^Tx_i)^2\ones\{g_i = 1\}\end{aligned}\right\}
\]
is the reweighted least squares cost function. \cite{shimodaira2000Improving,byrd2019What,sagawa2019Distributionally}. We note that reweighing requires knowledge of the sensitive attribute, so its applicability is limited to problems in which the sensitive attribute is observed during training.

In the overparameterized case, we consider the ridgeless reweighted least squares estimator: $\tbeta_{\min} \triangleq \lim_{\lambda\searrow 0}\tbeta_{\lambda}$, where
\[\textstyle
\tbeta_{\lambda} \in \argmin_{\beta\in\reals^d}\tilde{R}(\beta) + \frac{\lambda}{2}\|\beta\|_2^2
\]
($\tilde{R}$ is the reweighted least squares cost function). This is motivated by empirical results that suggest the effect of reweighing diminishes during training, but $\ell_2$ regularization restores some of its intended effect \cite{byrd2019What,sagawa2019Distributionally}.

\subsection{Majority group subsampling} 

It is known that models trained by ERM may perform poorly on minority groups \cite{sagawa2019Distributionally}. One promising way of improving performance on minority groups is majority group subsampling--randomly discarding training samples from the majority group until the two groups are equally represented in the remaining training data. This achieves an effect similar to that of upweighing the loss on minority groups in the underparameterized regime.

% The goal of subsampling is similar to that of reweighing, but instead of upweighing the loss on the minority group, subsampling simply discards training samples from the majority group until the proportion of samples from the majority and minority groups are comparable. 

In the underparameterized case ($n > d$), reweighing is more statistically efficient (it does not discard training samples), so subsampling is rarely used. On the other hand, in the overparameterized case, reweighing may not have the intended effect on the performance of overparameterized models in minority groups \cite{byrd2019What}, but \citet{sagawa2020Investigation} show that subsampling does. Thus we also consider subsampling here as a way of improving performance in minority groups. 
% We note that subsampling, like reweighing, requires access to the protected attribute, so its applicability is similarly limited.
We note that reweighing requires knowledge of the sensitive attribute, so its applicability is limited to problems in which the sensitive attribute is observed during training.

\paragraph{Hidden linearity in overparameterized neural networks} At this point, an astute reader may wonder whether fitting linear models is relevant to modern ML practice. There is a line of work that shows the training dynamics of overparameterized neural networks are similar to that of linear models \cite{jacot2018Neural,du2018Gradient,allen-zhu2018Convergence}. In particular, training only moves the weights of overparameterized neural networks by a small amount from their initial values, so the trained neural network is well approximated by the linearization around the initial weights:
\[
f(x;\widehat{w}) \approx f(x,w_0) + \partial_wf(x,w_0)^T(\widehat{w} - w_0),
\]
where $w_0$ and $\widehat{w}$ are vectors of initial and final weights. Further, the initial weights are often chosen randomly in a way such that $f(x,w_0) \approx 0$, so the trained network is approximately a linear model with the (random) features $\partial_wf(x,w_0)$. This connection between linear regression and overparameterized neural networks has been leveraged to study the generalization error of such neural networks \cite{hastie2019Surprises,mei2019generalization}. In this paper, we leverage this connection to study the performance of overparameterized neural networks on minority groups.


==> setup+theory.tex <==
\section{Setup} 

Consider an overparameterized linear regression problem. To keep things simple, we consider a two group setup: $g\in\{0,1\}$. WLOG we assume $\pi > \frac12$ (so the $g=1$ group is the majority group). The distribution of the training examples $\{(x_i,y_i)\}_{i=1}^n$ is
\begin{equation}
\begin{aligned}
g_i &\sim \Ber(\pi) \\
x_i &\sim N(0,\Sigma) \\
y_i\mid x_i,g_i &\gets (\beta_0 + \ones\{g_i=1\}\delta)^Tx_i + \eps_i,\quad\eps_i\sim N(0,\sigma^2)
\end{aligned},
\label{eq:two-groups}
\end{equation}
where $\Sigma\in\symm_+^d$ is a covariance matrix and $\beta_0,\delta\in\reals^d$ are vectors of regression coefficients. Here $\beta_0$ is the regression vector of the minority group and $\delta$ is the difference between the regression vectors of the majority and minority groups. 


\section{Unfairness of the minimum norm least squares estimator}

In the overparameterized setting ($n < d$), we consider the minimum norm least squares estimator
\begin{equation}
\hbeta \in \left\{\begin{aligned}&\argmin_{\beta\in\reals^d} & &\textstyle \frac12\|\beta\|_2^2 \\
& \st & & X\beta = y
\end{aligned}\right\} = X^\dagger y,
\label{eq:SVM}
\end{equation}
where $X\in\reals^{n\times d}$ is the feature matrix and $y\in\reals^n$ is the vector of responses. We wish to study the prediction error (MSPE) of $\hbeta$ on the minority group:
\[
\MSPE_0(\hbeta) \triangleq \Ex\big[((\hbeta - \beta_0)^Tx_{n+1})^2\big] = \Ex\big[(\hbeta - \beta_0)^T\Sigma(\hbeta - \beta_0)\big].
\]
To keep things simple, we assume $\Sigma = I_d$ for now. WLOG we arrange the training examples so that the first $n_0$ examples are from the minority group:
\[
X = \begin{bmatrix} X_0 \\ X_1\end{bmatrix},\quad y = \begin{bmatrix} y_0 \\ y_1\end{bmatrix}.
\]
The estimation error $\hbeta - \beta_0$ is
\[
\begin{aligned}
\hbeta - \beta_0 &\triangleq X^\dagger(X\beta_0 + \begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + \eps) - \beta_0 = (\Pi_X - I_d)\beta_0 + X^\dagger\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + X^\dagger\eps,
\end{aligned}
\]
where $\Pi_X \triangleq X^\dagger X$ is the (orthogonal) projector onto $\ran(X^T)$. The MSPE is
\begin{equation}
\begin{aligned}
&\Ex\big[(\hbeta - \beta_0)^T(\hbeta - \beta_0)\big] \\
&\quad= \beta_0^T\Ex\big[(I_d - \Pi_X)\big]\beta_0 + \delta^T\Ex\big[\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}^T(XX^T)^{-1}\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\big]\delta + \Ex\big[\eps^T(XX^T)^{-1}\eps\big].
\end{aligned}
\label{eq:MSPE}
\end{equation}
The first two terms on the right side are (squared) bias terms, and the third term is a variance term. The first bias term is due to the inductive bias of the minimum norm least squares estimator. It is possible to show that the first term on the right side of \eqref{eq:MSPE} is $(1-\frac{1}{\gamma})\|\beta_0\|_2^2$, where $\gamma \triangleq \frac{d}{n}$ is the aspect ratio, and third term is $\frac{\sigma^2}{\gamma - 1}$  (see Lemmas 2 and 3 in \cite{hastie2019Surprises}). 

In the rest of this section, we focus on evaluating the second bias term. This term is due to the difference between the majority and minority groups. We start by simplifying the matrix inside expectation in the second term. Let $\hSigma_0 \triangleq X_0^TX_0$. We have
\[
\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}^T(XX^T)^{-1}\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix} = X_1^T(X_1(I - X_0^\dagger X_0)X_1^T)^{-1}X_1 \]
\YK{This part is wrong. See subsection \ref{sec:bias}} We recognize this matrix as the product of  $\Pi_{X_1}$ and $(I_d - \Pi_{X_0})^\dagger$. We replace $\Pi_{X_1}$ with $\frac{n_1}{d}$ and $I_d - \Pi_{X_0}$ with $1-\frac{n_0}{d}$ to obtain
\begin{equation}
X_1^T(X_1X_1^T - X_1X_0^T(X_0X_0^T)^{-1}X_0X_1^T)^{-1}X_1 \approx \frac{\frac{n_1}{d}}{1 - \frac{n_0}{d}} \approx \frac{\pi/\gamma}{1-(1-\pi)/\gamma}.
\label{eq:ansatz}
\end{equation}
Thus the second bias term is $\frac{\pi/\gamma}{1-(1-\pi)/\gamma}\|\delta\|_2^2$. We see that this term grows as $\pi \nearrow 1$ (size of minority group decreases) and as $\gamma$ shrinks (the model is less overparameterized). This suggests overparameterization + $\ell_2$ regularization as a way to reduce this bias term.

\subsection{Evaluating the bias term carefully}
\label{sec:bias}

\begin{lemma} Let $d > n+1.$ If the generic covariate $x \sim N_d(0, I_d)$ then 
\[\Ex \big[\text{Bias}\big] =\|\delta\|_2^2 \left[ \frac{n_0n_1}{d(d-n-1)} + \frac{n_1}{d}\right].\]
\end{lemma}

The main takeaway this result is the limiting bias due to the difference between the regression vectors has the form
\begin{equation}
\|\delta\|_2^2(\frac{n_0}{d}\frac{n_1}{d-n-1} + \frac{n_1}{d}) \approx \|\delta\|_2^2( \frac{1-\pi}{\gamma}\frac{\pi}{\gamma - 1} + \frac{\pi}{\gamma}),
\label{eq:limiting-bias}
\end{equation}
where recalled $\gamma = \frac{d}{n}$ and $\pi\approx\frac{n_1}{n}$. We see that the bias increases as $\pi$ increases. This is unsurprising. (i) the bias increase as $\pi$ increases, and (ii) the bias decreases as $\gamma$ increaese. The former is unsurprising: we expect the bias to increase as the fraction of minority examples decreases. The latter is surprising: it seems to contradict the empirical results in \cite{sagawa2020Investigation}. However, the prediction error \eqref{eq:MSPE} may still increase as $\gamma$ grows. Combining (this approximation of)  \eqref{eq:limiting-bias} and the limits of the first and third terms in \eqref{eq:MSPE}, we see that the limiting prediction error is
\[
(1-\frac1\gamma)\|\beta_0\|_2^2 + \Ex[Bias] + \frac{\sigma^2}{\gamma-1} \approx \|\beta_0\|_2^2 + (\|\delta\|_2^2\pi - \|\beta_0\|_2^2 + \sigma^2)\frac1\gamma.
\]
As long as the coefficient in front of the $\frac1\gamma$ term is negative, then the prediction error may increase as $\gamma$ increases.


\begin{proof}
Without loss of generality assume $\|\delta\|_2 = 1.$ Note that $\bI - \Pi_{X_0'} = \bI - X_0' (X_0X_0')^{-1} X_0$ is idempotent symmetric with rank $d-n_0.$ Then we have the following  spectral decomposition $\bI - \Pi_{X_0'} = P\Lambda P'$ where $P$ is a $d\times d$ orthogonal matrix and $\Lambda$ is diagonal matrix with \[ (\Lambda)_{ii} = \begin{cases} 1 & \quad \text{if } 1\le i \le d-n_0\\
0 & \quad \text{otherwise.}\end{cases}\] We define $\Ex_1 = \Ex_{X_1}$ and $\Ex_0 = \Ex_{X_0}.$
Let $\xi = P'\delta$, $Y = X_1P = [Y_1, \dots, Y_d].$ Note that $Y_1, \dots, Y_d \sim \iid\  N_{n_1}(0, \bI_{n_1}).$

\[
\begin{aligned}
\text{Bias} = & \delta' X_1' \Big( X_1 (\bI - \Pi_{X_0'}) X_1'   \Big)^{-1} X_1 \delta \\
 = & \delta' P P' X_1' \big( X_1 P \Lambda P' X_1' \big)^{-1} X_1PP' \delta \\
 = & \xi' Y'  \big(Y \Lambda Y' \big)^{-1} Y \xi\\
 = & \Big(\sum_{i=1}^d \xi_i Y_i\Big)^T \Big(\sum_{i=1}^{d-n_0} Y_iY_i^T\Big)^{-1} \Big(\sum_{i=1}^{d} \xi_i Y_i\Big) \\
 = & \underbrace{\Big(\sum_{i=1}^{d-n_0} \xi_i Y_i\Big)^T \Big(\sum_{i=1}^{d-n_0}  Y_iY_i^T\Big)^{-1} \Big(\sum_{i=1}^{d-n_0} \xi_i Y_i\Big)}_{(A)}\\
 &+  \underbrace{2\Big(\sum_{i=1}^{d-n_0} \xi_i Y_i\Big)^T \Big(\sum_{i=1}^{d-n_0}  Y_iY_i^T\Big)^{-1} \Big(\sum_{i=d - n_0+1}^{d} \xi_i Y_i\Big)}_{(B)}\\
 &+  \underbrace{\Big(\sum_{i=d - n_0+1}^{d} \xi_i Y_i\Big)^T \Big(\sum_{i=1}^{d-n_0}  Y_iY_i^T\Big)^{-1} \Big(\sum_{i=d - n_0+1}^{d} \xi_i Y_i\Big)}_{(C)}\\
\end{aligned}
\]

\noindent \textbf{(C)}
We note that \[ \left\{\begin{aligned}
& \sum_{i=d - n_0+1}^{d} \xi_i Y_i \sim  \left(\sum_{i=d - n_0+1}^{d} \xi_i^2 \right)   N_{n_1} (0, \bI_{n_1})\\
& \sum_{i=1}^{d-n_0}  Y_iY_i^T \sim \text{Wishart}(\bI_{n_1}, d-n_0)\\
& \sum_{i=d - n_0+1}^{d} \xi_i Y_i \text{ and } \sum_{i=1}^{d-n_0}  Y_iY_i^T \text{ are independent.}
\end{aligned}\right. \] Hence, \[ \text{(C)} = \left(\sum_{i=d - n_0+1}^{d} \xi_i^2 \right) \frac{T^2(d-n_0, n_1)}{d-n_0} = \left(\sum_{i=d - n_0+1}^{d} \xi_i^2 \right) \frac{\frac{(d-n_0)n_1}{d-n_0-n_1+1}F(n_1, d-n_0-n_1+1)}{d-n_0} \] and \[ 
\begin{aligned}
\Ex_1[\text{(C)}] =&  \left(\sum_{i=d - n_0+1}^{d} \xi_i^2 \right) \frac{n_1}{d-n+1} \Ex\left[F(n_1, d-n+1)\right]\\
= & \left(\sum_{i=d - n_0+1}^{d} \xi_i^2 \right) \frac{n_1}{d-n+1}\frac{d-n+1}{d-n-1}\\
=& \left(\sum_{i=d - n_0+1}^{d} \xi_i^2 \right) \frac{n_1}{d-n-1}.
\end{aligned}
   \]
   
   
   \noindent \textbf{(B)} \[
   \begin{aligned}
   \Ex_1[\text{B}] &= \Ex\left[ 2\Big(\sum_{i=1}^{d-n_0} \xi_i Y_i\Big)^T \Big(\sum_{i=1}^{d-n_0}  Y_iY_i^T\Big)^{-1} \Big(\sum_{i=d - n_0+1}^{d} \xi_i Y_i\Big) \right]\\
   &= \Ex\left[ 2\Big(\sum_{i=1}^{d-n_0} \xi_i Y_i\Big)^T \Big(\sum_{i=1}^{d-n_0}  Y_iY_i^T\Big)^{-1}\right]\Ex\left[ \Big(\sum_{i=d - n_0+1}^{d} \xi_i Y_i\Big) \right]\\
   &= 0.
   \end{aligned}
   \]
   
   
   \noindent \textbf{(A)} Let $u = (\xi_1, \dots, \xi_{d-n_0})^T/\sqrt{\sum_{i=1}^{d-n_0}  \xi_i^2}$ and $Q$ is $(d-n_0)\times (d-n_0) $ an orthogonal matrix with first column $u$. Define $Z = YQ = [Z_1, \dots, Z_{d-n_0}].$ Then $Z_1, \dots, Z_{d-n_0} \sim \iid\ N_{n_1}(0, \bI_{n_1}).$
   
   \[ \begin{aligned}
   \text{(A)} =&  \Big(\sum_{i=1}^{d-n_0} \xi_i Y_i\Big)^T \Big(\sum_{i=1}^{d-n_0}  Y_iY_i^T\Big)^{-1} \Big(\sum_{i=1}^{d-n_0} \xi_i Y_i\Big) \\
   =& \left(\sum_{i=1}^{d-n_0}  \xi_i^2\right) Z_1^T \Big(\sum_{i=1}^{d-n_0}  Z_iZ_i^T\Big)^{-1}Z_1 \\
= & \left(\sum_{i=1}^{d-n_0}  \xi_i^2\right) Z_1^T \left(Z_1Z_1^T + \sum_{i=2}^{d-n_0}  Z_iZ_i^T\right)^{-1}Z_1\\
= & \left(\sum_{i=1}^{d-n_0}  \xi_i^2\right) \left[ Z_1^T \left(\sum_{i=2}^{d-n_0}  Z_iZ_i^T\right)^{-1}Z_1 - \frac{\left(Z_1^T \left(\sum_{i=2}^{d-n_0}  Z_iZ_i^T\right)^{-1}Z_1\right)^2 }{1+ Z_1^T \left(\sum_{i=2}^{d-n_0}  Z_iZ_i^T\right)^{-1}Z_1} \right] \\
& \quad \text{using } (A+ab')^{-1} = A^{-1} - \frac{A^{-1}ab' A^{-1}}{ 1+ b' A^{-1}a}, \\
= & \left(\sum_{i=1}^{d-n_0}  \xi_i^2\right) \frac{Z_1^T \left(\sum_{i=2}^{d-n_0}  Z_iZ_i^T\right)^{-1}Z_1 }{1+ Z_1^T \left(\sum_{i=2}^{d-n_0}  Z_iZ_i^T\right)^{-1}Z_1}
   \end{aligned}  \]
Since 
\[\left\{ \begin{aligned}
& Z_1 \sim N_{n_1} (0, \bI_{n_1})\\
& \sum_{i=2}^{d-n_0}  Z_iZ_i^T \sim \text{Wishart}(\bI_{n_1}, d-n_0-1)
\end{aligned}\right. \] we have 
\[
\begin{aligned}
Z_1^T \left(\sum_{i=2}^{d-n_0}  Z_iZ_i^T\right)^{-1}Z_1 &= \frac{T^2(d-n_0-1, n_1)}{d-n_0-1}\\
&= \frac{\frac{n_1(d-n_0-1)}{d-n_0-n_1}F(n_1, d-n_0-n_1)}{d-n_0-1}\\
&= \frac{n_1}{d-n}F(n_1, d-n)\\
&= \frac{\chi^2(n_1)}{\chi^2(d-n)}.
\end{aligned}
  \]
  This implies \[ \begin{aligned}
  \text{(A)} =& \left(\sum_{i=1}^{d-n_0}  \xi_i^2\right) \frac{\frac{\chi^2(n_1)}{\chi^2(d-n)}}{1+\frac{\chi^2(n_1)}{\chi^2(d-n)}}\\
  =& \left(\sum_{i=1}^{d-n_0}  \xi_i^2\right) \frac{\chi^2(n_1)}{\chi^2(n_1) + \chi^2(d-n)}\\
    =& \left(\sum_{i=1}^{d-n_0}  \xi_i^2\right) \frac{\text{Gamma}\left(\frac{n_1}2, \frac12\right)}{\text{Gamma}\left(\frac{n_1}2, \frac12\right) + \text{Gamma}\left(\frac{d-n}2, \frac12\right)}\\
  =& \left(\sum_{i=1}^{d-n_0}  \xi_i^2\right) \text{Beta} \left(\frac{n_1}{2}, \frac{d-n}{2} \right)
  \end{aligned} \]
  and, \[\Ex_1 [\text{(A)}] = \left(\sum_{i=1}^{d-n_0}  \xi_i^2\right) \Ex \left[\text{Beta} \left(\frac{n_1}{2}, \frac{d-n}{2} \right)\right] =  \left(\sum_{i=1}^{d-n_0}  \xi_i^2\right) \frac{n_1}{d-n+n_1} = \left(\sum_{i=1}^{d-n_0}  \xi_i^2\right) \frac{n_1}{d-n_0}. \]
  
  It can be argued from direction invariance of $N_d(0, \bI_d)$ that $\Ex_0 [\xi_i^2] = \frac 1d.$ [Argue that the projection space formed by $X_0$ in $\reals^d$ is uniformly distributed on the set of all $n_0$ dimensional projection spaces in $\reals^d$ (whatever that is), and $\sum_{i=1}^d \xi_i^2 = 1.$ ] Hence, we have the result. 
\end{proof}

\section{MSE for under-parameterizatized setting}
In the under-parameterized setting ($n>d$), we consider the least square estimator \[ \hat \beta = (X^TX)^{-1}X^Ty. \]
\begin{theorem}
Let $n, p \to \infty $ with $p/n\to \gamma \in (0, 1).$ Then \[
\text{MSPE} = \frac{\sigma^2 \gamma}{1-\gamma} + \frac{\pi\gamma\|\delta\|^2}{1-\gamma} + \frac{\pi^2 (1-2\gamma)\|\delta\|^2}{1-\gamma}. \]
\end{theorem}
\begin{proof}




The estimation error is \[
\begin{aligned}
\hat \beta - \beta_0 & =  (X^TX)^{-1}X^T(X\beta_0 + \begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + \eps) - \beta_0\\
& = (X^TX)^{-1}X^T\begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta + (X^TX)^{-1}X^T\eps
\end{aligned}
 \]
The MSPE is \[
\begin{aligned}
& \Ex\big[ (\hat \beta - \beta_0)^T(\hat \beta - \beta_0) \big]\\
& \quad = \Ex \left[ \delta^T \begin{bmatrix} 0_{n_0\times d} , X_1^T\end{bmatrix} X (X^TX)^{-2}X^T \begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta \right] + 2\Ex \big[ \delta^T \begin{bmatrix} 0_{n_0\times d}  X_1\end{bmatrix} X (X^TX)^{-2}X^T \eps \big]\\
& \quad \quad + \Ex \big[ \eps^T X(X^TX)^{-2}X^T\eps \big]
\end{aligned}
\]



To calculate the variance term we see that \[
\begin{aligned}
& \Ex \big[ \eps^T X(X^TX)^{-2}X^T\eps \big]\\
& \quad = \Ex \text{Tr}\big[ X(X^TX)^{-2}X^T\Ex_\eps(\eps \eps^T) \big]\\
& \quad = \sigma^2\Ex \text{Tr}\big[ (X^TX)^{-2}X^TX \big] \\
& \quad = \sigma^2\Ex \text{Tr}\big[ (X^TX)^{-1} \big] \\
& \quad = \sigma^2\frac{p}{n}\frac{1}{p}\Ex \text{Tr}\big[ (X^TX/n)^{-1} \big] \\
& \quad \to \sigma^2 \gamma \int \frac{1}{s}d\mu_\gamma(s)\\
&\quad = \frac{\sigma^2 \gamma}{1-\gamma}
\end{aligned}
\]
The covariance term $\Ex \big[ \delta^T \begin{bmatrix} 0_{n_0\times d}  X_1\end{bmatrix} X (X^TX)^{-2}X^T \eps \big]$ is zero. 

We now focus on the bias term. Note that, 
\[ \Ex \left[ \delta^T \begin{bmatrix} 0_{n_0\times d}  X_1^T\end{bmatrix} X (X^TX)^{-2}X^T \begin{bmatrix} 0_{n_0\times d} \\ X_1\end{bmatrix}\delta \right] = \Ex \left[ \delta^T X_1^TX_1 (X^TX)^{-2}X_1^TX_1 \delta \right] \]
and for any $p \times p  $ orthogonal matrix $U$ \[ \Ex \left[ \delta^T X_1^TX_1 (X^TX)^{-2}X_1^TX_1 \delta \right] = \Ex \left[ \delta^TU^T X_1^TX_1 (X^TX)^{-2}X_1^TX_1 U\delta \right] \]
Letting $U$ be such an orthogonal matrix that $U\delta = \|\delta \|_2^2 e_i$ and averaging over $i = 1, 2, \dots, p$ we get \[
\begin{aligned}
\text{BIAS} &= \frac{\|\delta \|_2^2}{p}\Ex\left[ \text{Tr}\left\{ (X_1^TX_1)(X^TX)^{-2}(X_1^TX_1) \right\}\right]\\
&= \frac{\|\delta \|_2^2}{p}\Ex\left[ \text{Tr}\left\{ \left(\sum_{i=1}^{n_1}x_ix_i^T\right)^2(X^TX)^{-2} \right\}\right]\\
&= \frac{\|\delta \|_2^2}{p}\Ex\left[ \text{Tr}\left\{ \left(\sum_{i=1}^{n_1}\sum_{j=1}^{n_1}x_ix_i^Tx_jx_j^T\right)(X^TX)^{-2} \right\}\right]\\
&= \frac{\|\delta \|_2^2}{p} \Big[ n_1 \Ex \big[x_1^Tx_1 x_1^T(X^TX)^{-2}x_1\big] + n_1(n_1-1) \Ex \big[x_1^Tx_2 x_1^T(X^TX)^{-2}x_2\big] \Big]\\
&= \frac{\|\delta \|_2^2}{p} \big[ n_1 D_1 + n_1(n_1-1) D_2 \big]
\end{aligned}
\]

where the second last equality is obtained using exchangeability of $x_i$'s.

Using the above logic we get 
\begin{equation}
\label{eq:equality-D_1-D_2}
    n D_1 + n(n-1) D_2 = \Ex\Big[ \text{Tr}\big\{ (X^TX)(X^TX)^{-2}(X^TX) \big\}\Big] = p
\end{equation}

Let $A = X^T - x_1x_1^T.$ Hence \[
\begin{aligned}
x_1^T (A+x_1x_1^T)^{-2} x_1 &= x_1 ^T \left( A^{-1} - \frac{A^{-1}x_1x_1^T A^{-1}}{1+ x_1^TA^{-1}x_1}  \right) \left( A^{-1} - \frac{A^{-1}x_1x_1^T A^{-1}}{1+ x_1^TA^{-1}x_1}  \right) x_1\\
& = x_1^T A^{-1} \left( 1- \frac{x_1^T A^{-1}x_1}{1+x_1^2 A^{-1}x_1} \right)^2 A^{-1}x_1\\
& = \frac{x_1^TA^{-2}x_1}{(1+x_1^TA^{-1}x_1)^2}
\end{aligned}
\]

and \[ 
\begin{aligned}
D_1 & = \Ex \left[\frac{x_1^TA^{-2}x_1 x_1^T x_1}{(1+x_1^TA^{-1}x_1)^2}\right] \\
& = \Ex\left[ \frac{\frac{p^2}{(n-1)^2}\Big( x_1^T (A/(n-1))^{-2}x_1/p \Big) \Big( x_1^Tx_1/p \Big) }{\Big(1+\frac{p}{n-1}\big(x_1^T (A/(n-1))^{-1}x_1/p\big)\Big)^2}\right]\\
& \to \frac{\gamma^2 /(1-\gamma)^3}{\left(1+\gamma/(1-\gamma)\right)^2} = \frac{\gamma^2}{1-\gamma}
\end{aligned}
\] where the limit is obtained using lemmas \ref{lemma:p-conv} and \ref{lemma:moments-mp}. 

Using the equality \eqref{eq:equality-D_1-D_2} we get \[
D_2 = \frac{p - nD_1}{n(n-1)} \asymp \frac{\gamma - \frac{\gamma^2}{1-\gamma}}{n}  = \frac{\gamma(1-2\gamma)}{n(1-\gamma)}.
\]
Finally, we get \[
\begin{aligned}
\text{BIAS} &= \frac{\|\delta \|_2^2}{p} \big[ n_1 D_1 + n_1(n_1-1) D_2 \big]\\
& = \|\delta \|_2^2 \left[ \frac{\pi}{\gamma} \frac{\gamma^2}{1-\gamma} + \frac{\pi^2 }{\gamma}\frac{\gamma(1-2\gamma)}{1-\gamma}  \right]\\
& = \|\delta \|_2^2  \frac{\pi}{1-\gamma} (\gamma + \pi(1-2\gamma))
\end{aligned}
\]




\end{proof}

\begin{lemma}
\label{lemma:p-conv}
As $n, p\to \infty $ with $p/n \to \gamma\in (0, 1)$
\[
x_1^T (A/(n-1))^{-j}x_1/p \stackrel{p}{\to}\int \frac 1{s^{j}} d\mu_\gamma (s).  \]
\end{lemma}
\begin{proof}
We have \[
\begin{aligned}
\Ex \Big( x_1^T (A/(n-1))^{-j}x_1/p \Big) & = \frac{1}{p} \text{Tr} \Big((A/(n-1))^{-j}\Big)\\
\to \int \frac 1{s^{j}} d\mu_\gamma (s)
\end{aligned}
\] and \[
\begin{aligned}
\textbf{Var} \Big( x_1^T (A/(n-1))^{-j}x_1/p \Big) & = \frac{2}{p^2} \text{Tr} \Big((A/(n-1))^{-2j}\Big)\\
& \asymp\frac1p \int \frac 1{s^{2j}} d\mu_\gamma (s) \to 0
\end{aligned}
\]
\end{proof}

\begin{lemma}
\label{lemma:moments-mp}
For $0\le \gamma\le 1$ let $X\sim \mu_\gamma$ be a  Marchenko-Pastur random variable. Then \[ \Ex [1/X] = \frac{1}{1-\gamma}, \quad \Ex [1/X^2 ] = \frac{1}{(1-\gamma)^3}. \]
\end{lemma}

\begin{proof}
The Stieltjes transformation of $\mu_\gamma$ is \[
\begin{aligned}
s_\gamma(z) =&  \int \frac{1}{x - z}d\mu_\gamma(x)\\
=& \frac{1-\gamma - z - \sqrt{(1-\gamma- z)^2 - 4\gamma z}}{2\gamma z}, \quad z \in \bbC\backslash [1-\sqrt{\gamma}, 1+\sqrt{\gamma}].
\end{aligned}
 \]
 
 For $|z|< 1- \sqrt{\gamma}$
 \[
 \begin{aligned}
 s_\gamma(z) =&  \int \frac{1}{x - z}d\mu_\gamma(x)\\
=& \int \frac{1}{x}\frac{1}{1 - z/x}d\mu_\gamma(x)\\
=& \int \frac{1}{x}\sum_{k=0}^\infty (z/x)^k  d\mu_\gamma(x)
 \end{aligned}
 \]
 
 Hence, we have \[ \lim_{z\to 0+} s_\gamma (z) = \Ex[1/X], \quad \lim_{z\to 0+} \frac{d}{dz}\big(s_\gamma (z)\big) = \Ex[1/X^2]. \]
 
 Now, \[
 \begin{aligned}
 &1-\gamma -  z-\sqrt{(1-\gamma- z)^2 - 4\gamma z}\\ &\quad= 1-\gamma -  z-\big( 1+\gamma^2 + z^2 - 2\gamma - 2z + 2\gamma z - 4\gamma z \big)^{1/2} \\
 &\quad= 1-\gamma -  z-\big( (1-\gamma)^2 + z^2  - 2z - 2\gamma z  \big)^{1/2}\\
 &\quad \asymp 1-\gamma -  z-(1-\gamma) \Big[1+ \frac{z^2 -2z-2\gamma z}{2(1-\gamma)^2} - \frac{(z^2 -2z-2\gamma z)^2}{8(1-\gamma)^4}\Big],\quad \text{for }z \to 0+ \\
 &\quad \asymp 1-\gamma -  z-(1-\gamma) \Big[1+ \frac{z^2 -2z-2\gamma z}{2(1-\gamma)^2} - \frac{z^2(1+\gamma)^2}{2(1-\gamma)^4}\Big],\quad \text{for }z \to 0+ \\
 & \quad= \frac{z^2(1+\gamma)^2}{2(1-\gamma)^3}  - \frac{z^2-4\gamma z}{2(1-\gamma)} \\
 & \quad = \frac{2z^2 \gamma}{(1-\gamma)^3} + \frac{2\gamma z}{1-\gamma}
 \end{aligned}
 \]
 
which implies \[
\begin{aligned}
s_\gamma(z) \asymp \frac{z}{(1-\gamma)^3} + \frac{1}{1-\gamma}
\end{aligned}
\]
 This proves the lemma. 
\end{proof}

